AdaLoss: A computationally-efficient and provably convergent adaptive gradient method

We propose a computationally-friendly adaptive learning rate schedule, "AdaLoss", which directly uses the information of the loss function to adjust the stepsize in gradient descent methods. We prove that this schedule enjoys linear convergence in linear regression. Moreover, we provide a linear convergence guarantee over the non-convex regime, in the context of two-layer over-parameterized neural networks. If the width of the first-hidden layer in the two-layer networks is sufficiently large (polynomially), then AdaLoss converges robustly \emph{to the global minimum} in polynomial time. We numerically verify the theoretical results and extend the scope of the numerical experiments by considering applications in LSTM models for text clarification and policy gradients for control problems.

==> SGD.tex <==
In the stochastic setting, instead of observing an average loss  and  full gradient, we observe the stochastic gradient of each sample, i.e., the
  \emph{stochastic gradient}  $\frac{\partial L_{\xi_k}(\vW(k))}{\partial \vw_{r}}$  at $k$ iteration:
%  \begin{align*}
%    \frac{\partial L_{
%    \xi_k}(\vW(k))}{\partial \vw_r} = \frac{1}{\sqrt{m}}
%     (u_{\xi_k}(k)-y_{\xi_k})\vx_{\xi_k}\mathbb{I}_{\{\vw_r^T\vx__{
%    \xi_k}\geq0\}}
% \end{align*} 
where the sample loss can be  expressed as 
 \begin{align*}
   L_{\xi_{k}}(\vW(k)) = 
     \frac{1}{2}( u_{\xi_k}(k)-y_{\xi_k})^2, \quad   u_{\xi_k}(k)=
      \frac{1}{\sqrt{m}}\sum_{r=1}^{m}a_r
     \sigma(\langle{\vw_r(k), \vx_{\xi_k} \rangle})
 \end{align*}
 Here $\xi_k$, $k = 0,1,2 \dots$ are random variables. \footnote{ $\mathbb{E}_{\xi_k}[\cdot ]$ means expectation over the random variable $\xi_k$ conditional on the random sequence $\{\xi_\ell\}_{\ell=1} ^{k-1}$, and $\mathbb{E}_{\xi_1,\cdots,\xi_k}[\cdot]$ over the  random sequence $\{\xi_\ell\}_{\ell=0}^k$.} The upper bound of the stochastic gradient is
\begin{align}
	\max_{r\in[m]} \norm{\frac{\partial L_{\xi_{k}}(\vW{(k)})}{\partial \vw_r}} = &\max_{r\in[m]}\norm{
	 \frac{1}{\sqrt{m}} (y_{\xi_k}-u_{\xi_k}(k))a_r\vx_{\xi_k}\mathbb{I}_{\{\vw_r(k)^\top \vx_{\xi_k} \ge 0\} } }_2
	 \nonumber\\
\le &\frac{1}{\sqrt{m}} |y_{\xi_k}-u_{\xi_k}(k)| \|\vx_{\xi_k}\|_2 \nonumber\\
\le &\frac{1}{\sqrt{m}}|y_{\xi_k}-u_{\xi_k}(k)| \label{eq:grad_bound}
\end{align}
% The update of  SGD and AdaGrad at iteration $j,  j= 0,1,\cdots$ are respectively
% \begin{algorithm}[H]
%   \caption{SGD with adaptive stepsize or constant stepsize} \label{alg:Adagrad}
% \begin{algorithmic}[1]
%   \State {\bfseries Input:} 
%   Initialize $\vW_0 \in \mathbb{R}^d, b_{0}>0, \eta>0, \alpha>0$, the total iterations $N$ and the tolerance $\epsilon$
%     \For{\texttt{ $j = 1,2, \ldots, N$ }}
%      \State Generate  $\xi_{j-1}$ and $G_{j-1} = \nabla L(\vW_{j-1}, \xi_{j-1})$
% %      \State${b}_{j}^2 \leftarrow  {b}_{j-1} ^2+ { \| G_{j-1} \|^2}$  
%       \State $\vW_{j} \leftarrow \vW_{j-1} -  \frac{\eta}{{b}_{j}}G_{j-1} $
%       \State Calculate $ L(\vw_j;\xi_{j-1}) $
%       \If{$ L(\vW_j;\xi_{j-1}) > \epsilon$}
%       \State AdaGrad-Norm: ${b}_{j}^2 \leftarrow  {b}_{j-1} ^2+  \alpha L(\vW_j;\xi_{j-1}); \quad$ SGD: ${b}_{j}=b_0$
%       \Else
%       \State Break
%   \EndIf
%       \EndFor
% \end{algorithmic}
%   \end{algorithm}
%
%  \begin{align*}
%  &1. \text{ Draw the random variable } \xi_k\\
%  &2. \text{ Calculate the stochastic loss }  L_{\xi_{k}}(\vW(k)) = \frac{1}{2}(u_{\xi_k}(k) - y_{\xi_k}(k))^2\\ 
% &3. \text{ SGD } \quad \vw_r(k+1)=  \vw_r(k) - \eta \frac{\partial L_{
%    \xi_k}(\vW(k))}{\partial \vw_r} \\
%  & \quad\text{AdaGrad } \quad \vw_r(k+1) =  \vw_r(k) - \frac{\eta}{b_{k+1}} \frac{\partial L_{
%    \xi_k}(\vW(k))}{\partial \vw_r}   \text{ with }  b_{k+1}^2 = b_{k}^2 + \alpha^2n |u_{\xi_k}(k) - y_{\xi_k}(k)|
%  \end{align*} 
 We make  following assumptions: for each $k \geq 0$,
 \begin{asmp} \label{asmp1}
 $\xi_k$, $k = 0,1,2, \dots, $ are i.i.d. and also independent of weight matrix $\vW(k)$; \footnote{Observe that $\vW(k)$ is random variable dependent on the sequence of $\{\xi_{\ell}\}_{\ell=0}^{k-1}$.}
 \end{asmp}
 \begin{asmp} \label{asmp2}$\frac{\partial  L_{\xi_k}(\vW(k))}{ \partial \vw_{r}}$ is an unbiased estimator of $\frac{\partial L_{\xi_k}(\vW(k))}{\partial \vw_{r}}$, i.e.,
 $$\mathbb{E}_{\xi_k}\left[ \frac{\partial L_{\xi_k}(\vW(k))}{\partial \vw_{r}}\right] = \frac{\partial  L(\vW(k))}{ \partial \vw_{r}};$$
\end{asmp}
 \begin{asmp} \label{asmp3} There exist a constant $\sigma_k$ such that \begin{align*}
\sum_{i=1}^n\mathbb{E}_{\xi_k}\left[\left( (u_{\xi_k}-y_{\xi_k})\mat{H}_{i\xi_k}(k) -\frac{1}{n}\sum_{j=1}^n(u_j-y_j)\mat{H}_{ij}(k) \right)^2\right] 	=  \sigma_k^2 < \infty
 \end{align*}
\end{asmp}
Drawing a sample $(x_{\xi_k},y_{\xi_k})$ equally with probability $\frac{1}{n}$ implies
$$ \mathbb{E}_{\xi_k}\left[(y_{\xi_k}-u_{\xi_k}(k))^2\right] = \frac{1}{n}  \|\vy - \vu(k)\|_2^2.$$
Thus, using the bound of \eqref{eq:grad_bound} gives
\begin{align}
\frac{1}{\sqrt{m}}\mathbb{E}_{\xi_k}\left[|y_{\xi_k}-u_{\xi_k}(k)|\right] 
=& \frac{1}{n\sqrt{m}}
\sum_{i=1}^n|y_{i}-u_{i}(k)|
 =   \frac{1}{\sqrt{m} }\frac{\| \vy - \vu(k)\|_2}{\sqrt{n}}
 \label{eq:sgd_grad_bound}
\end{align}

\textbf{Theorem \ref{thm:main_sgd}}\textbf{(Convergence Rate of Stochastic Gradient Descent)}
Under the same setting as \cite{du2018gradient}, and standard  assumptions of the SGD algorithms (See Assumptions  \ref{asmp1},  \ref{asmp2}  and  \ref{asmp3}). 
% \simon{What is the $m$ dependency?}
Each sample $(x_{\xi_k},y_{\xi_k})$ is uniformly chosen with probability $\frac{1}{n}$. With over-parametrization $
m = \Omega \left(\frac{n^8}{\lambda_0^4\delta^3\widetilde{\delta}}  \right)$ with high probability $1-\widetilde{\delta}$ , 
% 	Set the stepsize 
% $ \eta = \Theta \left ( \frac{1}{ \norm{\vH^{\infty}}} \right),$
%  then with probability at least $1-\delta$
%  over the random initialization, after
% $T =\widetilde{O} \left({ \norm{ \vH^{\infty}}} \log\left( { 1 }/{ \varepsilon} \right)/{   \lambda_0 } \right) \text{ iterations, we have }
% L(\mat{W}(T)) \le \varepsilon + \sum_{k=0}^{T}\left( 1-\frac{\lambda_0}{\|\vH^{\infty}\|}\right)^{k} \sigma_{T-k}+c. 
% $
if we set the stepsize to be 
$ \eta = O \left ( \frac{\lambda_0}{n} \right),$
 then with probability at least $1-\delta-\delta'$, after
$
T =\widetilde{O} \left( \frac{n^2}{   \lambda_0^2\delta' } \log\left( \frac{ 1 }{ \varepsilon} \right) \right)\text{ iterations, we have }
 L(\mat{W}(T)) \le \varepsilon. 
$

\begin{proof}
Define the event \[A_{ir} = \left\{\exists \vect{w}: \norm{\vect{w}-\vect{w}_r(0)} \le R, \indict\left\{\vect{x}_i^\top \vect{w}_r(0) \ge 0\right\} \neq \indict\left\{\vect{x}_i^\top \vect{w} \ge 0\right\} \right\} \quad \text{ with } 
R= \frac{c \lambda_0 \delta}{n^2}\]
for some small positive constant $c$.

We let
$S_i = \left\{r \in [m]: \indict\{A_{ir}\}= 0\right\}$ and $
S_i^\perp = [m] \setminus S_i$.
 The following lemma bounds the sum of sizes of $S_i^\perp$.
\begin{lem}\label{lem:bounds_Si_perp}
With probability at least $1-\delta$ over initialization, we have $\sum_{i=1}^{n}\abs{S_i^\perp} \le  \frac{C_2mnR}{\delta}$  for some positive constant $C_2$.
\end{lem}
Next, we calculate the difference of predictions between two consecutive iterations,
\begin{align}
[\vu(k+1)]_i - [\vu(k)]_i 
= & \frac{1}{\sqrt{m}}\sum_{r=1}^{m} a_r \left(\relu{\left(
	\vect{w}_r(k) - \eta\frac{\partial L_{\xi_k}(\mat{W}(k))}{\partial \vect{w}_r(k)}
	\right)^\top \vect{x}_i} - \relu{\vect{w}_r(k)^\top \vect{x}_i}\right) \nonumber\\
	=&  \eta \left( [\vect{Q}({\xi_k})]_i+\widetilde{[\vect{Q}}({\xi_k}]_i) \right)
	\label{eq:defineQQ}
\end{align}
where we divide the right-hand side into two parts such that
$[\vect{Q}({\xi_k})]_i$  accounts for terms that the pattern does not change and $[\widetilde{\vect{Q}}({\xi_k})]_i$ accounts for terms that the pattern may change.
 Because $R' < R$, we know $\indict\left\{\vect{w}_r(k+1)^\top \vect{x}_i\ge 0\right\} \cap S_{i}= \indict\left\{\vect{w}_r(k)^\top \vect{x}_i \ge 0\right\}\cap S_{i}$.
\begin{align}
[\vect{Q}({\xi_k})]_i & \triangleq  \frac{1}{ \eta \sqrt{m}}\sum_{r \in S_i} a_r \left(\relu{\left(
	\vect{w}_r(k) - \eta\frac{\partial L_{\xi_k}(\mat{W}(k))}{\partial \vect{w}_r(k)}
	\right)^\top \vect{x}_i} - \relu{\vect{w}_r(k)^\top \vect{x}_i}\right) \nonumber\\
	&= -\frac{1}{\sqrt{m}} \sum_{r \in S_i} a_r \langle{ \frac{\partial L_{\xi_k}(\mat{W}(k))}{\partial \vect{w}_r(k)}, \vx_i \rangle} \nonumber\\
	&=  - \left(u_{\xi_{k}}(k)-y_{\xi_{k}}\right)(\mat{H}_{i \xi_{k}}(k) -\mat{H}_{i \xi_{k}}^\perp(k)) \label{eq:defineQ1}\\
\Rightarrow  \quad 
\mathbb{E}_{\xi_k}\left[[\vect{Q}({\xi_k})]_i\right]  &= -\frac{1}{ nm}\sum_{j=1}^{n}\vect{x}_i^\top \vect{x}_j \left(u_j-y_j\right)\sum_{r \in S_i} \indict\left\{\vect{w}_r(k)^\top \vect{x}_i \ge 0, \vect{w}_r(k)^\top \vect{x}_j\ge 0 \right\}\nonumber\\
&=  -\frac{1}{n}\sum_{j=1}^{n}(u_j-y_j)(\mat{H}_{ij}(k) -\mat{H}_{ij}^\perp(k))\nonumber
\end{align}
where $
\mat{H}_{ij}^\perp(k) = \frac{1}{m}\sum_{r \in S_i^\perp}\vect{x}_i^\top \vect{x}_j \indict\left\{\vect{w}_r(k)^\top \vect{x}_i \ge 0, \vect{w}_r(k)^\top \vect{x}_j \ge 0\right\}
$ is a perturbation matrix. With high probability, we obtain an upper bound of the operator norm\begin{align*}
\norm{\mat{H}^\perp(k)}_2 \le \sum_{(i,j)=(1,1)}^{(n,n)} \abs{\mat{H}_{ij}^\perp (k)}
\le \frac{n \sum_{i=1}^{n}\abs{S_i^\perp}}{m}
\le   \frac{n^2 mR}{m} 
\le  n^2R.
\end{align*}
As for $[\widetilde{\vect{Q}}({\xi_k})]_i$, we have
\begin{align}
\mathbb{E}_{\xi_k}\left[[\widetilde{\vect{Q}}({\xi_k})]_i \right]
&\leq \mathbb{E}_{\xi_k}\left[ \frac{ |S_{i}^\perp|}{ \sqrt{m}}\abs{\bigg \langle{ \frac{\partial L_{\xi_k}(\mat{W}(k))}{\partial \vect{w}_r(k)}, \vx_i \bigg\rangle}} \right]  \le  \frac{  |S_{i}^\perp|}{ m} \mathbb{E}_{\xi_k}\left[ |y_{\xi_k}-u_{\xi_k}(k)| \right] \label{eq:defineQ2}\\
\Rightarrow  \mathbb{E}_{\xi_k}\left[[\widetilde{\vect{Q}}({\xi_k})]_i \right] &\leq \frac{ |S_{i}^\perp|  }{ \sqrt{m}} \frac{1}{n} \sum_{j=1}^n |y_{j}-u_{j}(k)|  \leq  \frac{  |S_{i}^\perp| \|\vy-\vu(k)\|  }{ m\sqrt{ n }}
\nonumber
%\\
%\Rightarrow  \mathbb{E}_{\xi_k}\left[\widetilde{Q}_i^2({\xi_k}) \right] &\leq  \frac{ |S_{i}^\perp|^2 \|\vy-\vu(k)\|^2  }{  n m}\nonumber
\end{align}
Similar to the classical analysis of gradient, we also need to bound the quadratic term,
\begin{align}
\mathbb{E}_{\xi_k}\left[\norm{\vect{u}(k+1)-\vect{u}(k)}_2^2\right]
&= \sum_{i=1}^n\mathbb{E}_{\xi_k}\left[\left(u_i(k+1)-u_i (k) \right)^2\right] \nonumber\\
&\leq \eta^2 \sum_{i=1}^n\mathbb{E}_{\xi_k}\left[\sum_{r=1}^m\abs{\bigg \langle{ \frac{\partial L_{\xi_k}(\mat{W}(k))}{\partial \vect{w}_r(k)}, \vx_i \bigg\rangle}}^2 \right]\nonumber\\
&\leq  \eta ^2  \sum_{i=1}^n \frac{1}{n} \sum_{j=1}^n |y_{j}-u_{j}(k)|^2 \nonumber\\
&\le  \eta^2  \norm{\vect{y}-\vect{u}(k)}^2. \label{eq:defineUU}
\end{align}

With these estimates at hand, we are ready to prove the induction hypothesis. That is, we bound $\mathbb{E}_{\xi_{k}}\left[\norm{\vect{y}-\vect{u}(k+1)}_2^2 \right]$ by the law of iterative conditional expectation,
\begin{align}
&\mathbb{E}_{\xi_{k}}\left[\norm{\vect{y}-\vect{u}(k+1)}^2 \right]\nonumber\\
= & \mathbb{E}_{\xi_{k}}\left[\norm{\vect{y}-\vect{u}(k) - (\vect{u}(k+1)-\vect{u}(k))}^2\right]\nonumber\\
= & \norm{\vect{y}-\vect{u}(k)}^2+ \mathbb{E}_{\xi_{k}}\left[\norm{\vect{u}(k+1)-\vect{u}(k)}^2\right] - 2 \left(\vect{y}-\vect{u}(k)\right)^\top \mathbb{E}_{\xi_{k}}\left[\left(\vect{u}(k+1)-\vect{u}(k)\right) \right]\nonumber\\
= & \norm{\vect{y}-\vect{u}(k)}^2+\mathbb{E}_{\xi_{k}}\left[\norm{\vect{u}(k+1)-\vect{u}(k)}^2\right]- \frac{2\eta}{n}  \left(\vect{y}-\vect{u}(k)\right)^\top \mat{H}(k) \left(\vect{y}-\vect{u}(k)\right)\nonumber\\
&+ \frac{2\eta}{n}  \left(\vect{y}-\vect{u}(k)\right)^\top \mat{H}(k)^\perp \left(\vect{y}-\vect{u}(k)\right) - \frac{2\eta}{n}  \left(\vect{y}-\vect{u}(k)\right)^\top \mathbb{E}_{\xi_k}\left[\widetilde{\vect{Q}}({\xi_k}) \right]\nonumber\\
\le & (1-\frac{\eta}{n} \lambda_0+ \eta^2 + 2\frac{\eta}{n} n^2R + 2\frac{\eta}{n}  n^{3/2} R ) \norm{\vect{y}-\vect{u}(k)}^2 \nonumber\\
\le & \left(1-\frac{\eta\lambda_0}{2n} \right)\norm{\vect{y}-\vect{u}(k)}^2 \label{eq:y-u1}
\end{align}
 where we have stepsize $\eta = O\left( \frac{\lambda_0}{n} \right)$ so that the convergence is guaranteed to reach zero.
 %However, we can use large learning rate $\eta = \theta\left( \frac{n}{\|\vH^{\infty}\|}\right)$ to have faster contraction up to a region bounded by the variance. To make the statement rigorous,  we use following analysis 
% \begin{align}
% &\mathbb{E}_{\xi_{k}}\left[\norm{\vect{y}-\vect{u}(k+1)}^2 \right]\nonumber\\
% = 
% & \mathbb{E}_{\xi_{k}}\left[\norm{\vect{y}- \left(\vect{u}(k) + \eta\vect{Q}(\xi_{k}) + \eta  \widetilde{\vect{Q}}({\xi_k}) \right)}^2 \right] \nonumber\\
% \leq &\norm{\vect{y}-\vect{u}(k)}^2 -  2\eta \left(\vect{y}-\vect{u}(k)\right)^\top\mathbb{E}_{\xi_{k}}\left[\vect{Q}(\xi_{k}) +\widetilde{\vect{Q}}({\xi_k}) \right]  \nonumber\\
% &+2\eta^2\mathbb{E}_{\xi_{k}}\left[\norm{\vect{Q}(\xi_{k})}^2\right]+2\eta^2\mathbb{E}_{\xi_{k}}\left[\norm{\widetilde{\vect{Q}}({\xi_k})}^2\right] \nonumber \\
% \leq &\norm{\vect{y}-\vect{u}(k)}^2 -  \frac{2\eta}{n}  \left(\vect{y}-\vect{u}(k)\right)^\top \left( \mat{H}(k) - \mat{H}(k)^\perp\right) \left(\vect{y}-\vect{u}(k)\right)  \label{eq:y-u2} \\
% &+2\eta^2\mathbb{E}_{\xi_{k}}\left[\norm{\vect{Q}(\xi_{k})}^2\right]+2\eta^2\mathbb{E}_{\xi_{k}}\left[\norm{\widetilde{\vect{Q}}({\xi_k})}^2\right] - \frac{2\eta \left(\vect{y}-\vect{u}(k)\right)^\top \mathbb{E}_{\xi_k}\left[\widetilde{\vect{Q}}({\xi_k}) \right]}{n} \nonumber
% \end{align}
% Plugging the variance of $\vect{Q}(\xi_{k})$ to \eqref{eq:y-u2}  recovers to \eqref{eq:y-u1} as  the variance of $\vect{Q}(\xi_{k})$ is
% \begin{align*}
% \mathbb{E}_{\xi_k}\left[ [\vect{Q}({\xi_k})]_i^2 \right] 	&\leq \frac{1}{m} |S_i| \sum_{r \in S_i} \mathbb{E}_{\xi_{k}}\left[ \abs{ \bigg\langle{ \frac{\partial L_{\xi_k}(\mat{W}(k))}{\partial \vect{w}_r(k)}, \vx_i \bigg\rangle} }^2\right] \\
% &\leq  \mathbb{E}_{\xi_{k}}\left[ \abs{y_{\xi_k} - u_{\xi_k} (k)}^2\right] \\
% &= \frac{1}{n} || \vy-\vu(k)||^2 \\
% \text{and} \quad  \mathbb{E}_{\xi_k}\left[ \|\vect{Q}(\xi_{k})\|^2\right] &\leq || \vy-\vu(k)||^2.
% \end{align*}
% On the other hand, if use Assumption (3), i.e.,
% \begin{align}
% &\mathbb{E}_{\xi_k}\left[ \|\vect{Q}(\xi_{k})-\frac{1}{n}\vect{H}(k) (\vy-\vu(k)) \|^2\right]\nonumber\\
% \leq& 2 \sum_{i=1}^n\mathbb{E}_{\xi_k}\left[\left( (u_{\xi_k}-y_{\xi_k})\mat{H}_{i\xi_k}(k) -\frac{1}{n}\sum_{j=1}^n(u_j-y_j)\mat{H}_{ij}(k) \right)^2\right] \\ &+2\sum_{i=1}^n \mathbb{E}_{\xi_k}\left[ (\mat{H}_{i \xi_{k}}^\perp(k) \left(u_{\xi_{k}}(k)-y_{\xi_{k}}\right))^2\right]\nonumber \\
% =&  2\sigma_k^2+\frac{2}{n}\sum_{i=1}^n \sum_{j=1}^n\left[ \left(\mat{H}_{ij}^\perp(k) (u_{j}(k)-y_{j})\right)^2\right]\nonumber \\
% \Rightarrow \quad & \mathbb{E}_{\xi_k}\left[ \|\vect{Q}(\xi_{k})\|^2\right] \leq 2\sigma_k^2 + \frac{1}{n^2}\|\vect{H}(k) (\vy-\vu(k))\|^2 + \frac{2}{n} \| \mat{H}^\perp(k)\|_{F}^2 \|\vu(k)-\vy\|^2
%  \label{eq:var} 
% \end{align}
% Then, we can use large learning rate $\eta = \frac{n}{\|\vH^{\infty}\|}$ to have faster contraction up to a region bounded by the sum of all the variance. To see why, let us plug \eqref{eq:var} back to \eqref{eq:y-u2}:
% \begin{align}
% &\mathbb{E}_{\xi_{k}}\left[\norm{\vect{y}-\vect{u}(k+1)}^2 \right]\nonumber\\
% \leq &\norm{\vect{y}-\vect{u}(k)}^2  -  \frac{2\eta}{n}\underbrace{\left(\vect{y}-\vect{u}(k)\right)^\top\left(\mathbf{I}-\frac{\eta}{2n}\mat{H}(k)\right) \mat{H}(k) \left(\vect{y}-\vect{u}(k)\right)}_{{Term 1}} +2\eta^2\sigma_k^2 \nonumber\\
% &+  \frac{2\eta}{n} \| \mat{H}^\perp(k)\|_{F} \left( \| \mat{H}^\perp(k)\|_{F}+1\right)\|\vect{y}-\vect{u}(k) \|^2+2\mathbb{E}_{\xi_{k}}\left[\norm{\widetilde{\vect{Q}}({\xi_k})}^2\right]\nonumber\\
% &- \frac{2\eta}{n}  \left(\vect{y}-\vect{u}(k)\right)^\top \mathbb{E}_{\xi_k}\left[\widetilde{\vect{Q}}({\xi_k}) \right]  \nonumber\\
% \leq & \left(1-\frac{2\eta\lambda_0}{n}\left( 1-\frac{\eta \|\vH(k)\|}{2n}\right) \right) \norm{\vect{y}-\vect{u}(k)}^2  +2\eta^2\sigma_k^2+ R(\widetilde{\vect{Q}}({\xi_k}) )  \nonumber \\
% = & \left(1-\frac{\lambda_0}{\|\vH^{\infty}\|} \right) \norm{\vect{y}-\vect{u}(k)}^2  +2\eta^2\sigma_k^2+ R(\widetilde{\vect{Q}}({\xi_k}) )  
% \end{align}

% where in the last inequality, we let 
% \begin{align*}
%   R(\widetilde{\vect{Q}}({\xi_k}) ) &=  \frac{2\eta}{n} \| \mat{H}^\perp(k)\|_{F} \left( \| \mat{H}^\perp(k)\|_{F}+1\right)\|\vect{y}-\vect{u}(k) \|^2+2\eta^2\mathbb{E}_{\xi_{k}}\left[\norm{\widetilde{\vect{Q}}({\xi_k})}^2\right]\\ 
% & \quad - \frac{2\eta}{n}  \left(\vect{y}-\vect{u}(k)\right)^\top \mathbb{E}_{\xi_k}\left[\widetilde{\vect{Q}}({\xi_k}) \right].
% \end{align*}
\input{rebuttal-sgd.tex}



\end{proof}
%\begin{theorem}[Convergence Rate of Stochastic Adaptive Gradient Descent]
%\label{thm:main_adagrad_sgd}
%Under the same assumptions and setting as Theorem \ref{thm:main_adagrad_sgd}.  Each sample $(x_{\xi_k},y_{\xi_k})$ is equally  chosen with probability $\frac{1}{n}$.  Then with high probability over the random initialization, we have $\mathbb{E}\left[(y_{\xi_{k}}-u_{\xi_{k}}(k))^2\right] \le \epsilon$.
% \end{theorem}
% \textbf{Proof:}
%The difference of predictions between two consecutive iterations is
%\begin{align*}
%u_{i}(k+1) - u_{i}(k) = &\frac{1}{n\sqrt{m}}\sum_{r=1}^{m} a_r \left(\relu{\vect{w}_r(k+1)^\top \vect{x}_{i}} - \relu{\vect{w}_r(k)^\top \vect{x}_{i}}\right)\\
%= & \frac{1}{n\sqrt{m}}\sum_{r=1}^{m} a_r \left(\relu{\left(
%	\vect{w}_r(k) -  \frac{\eta}{b_{k+1}}\frac{\partial L_{\xi_k}(\mat{W}(k))}{\partial \vect{w}_r(k)}
%	\right)^\top \vect{x}_{i}} - \relu{\vect{w}_r(k)^\top \vect{x}_{i}}\right).
%\end{align*}
%Here we divide the right hand side into two parts.
%$I_1^{i}$ accounts for terms that the pattern does not change and $I_2^{i}$ accounts for terms that pattern may change.
%\begin{align*}
%I_1^{i} \triangleq  &\frac{1}{n\sqrt{m}}\sum_{r \in S_{i}} a_r \left(\relu{\left(
%	\vect{w}_r(k) - \frac{\eta}{b_{k+1}}\frac{\partial L_{\xi_k}(\mat{W}(k))}{\partial \vect{w}_r(k)}
%	\right)^\top \vect{x}_{i}} - \relu{\vect{w}_r(k)^\top \vect{x}_{i}}\right) \\
%I_2^{i} \triangleq &\frac{1}{n\sqrt{m}}\sum_{r \in S_{i}^\perp} a_r \left(\relu{\left(
%	\vect{w}_r(k) -\frac{\eta}{b_{k+1}}\frac{\partial L_{\xi_k}(\mat{W} (k))}{\partial \vect{w}_r(k)}
%	\right)^\top \vect{x}_{i}} - \relu{\vect{w}_r(k)^\top \vect{x}_{i}}\right)
%\end{align*}
%We view $I_2^{i}$ as a perturbation and bound its magnitude.
%Because ReLU is a $1$-Lipschitz function and $\abs{a_r}  =1$, we have 
%\begin{align*}
%\abs{I_2^{i}} 
%&\le \frac{\eta}{n\sqrt{m}b_{k+1}} \sum_{r\in S_{i}^\perp} \abs{\left(
%\frac{\partial L_{\xi_k}(\mat{W}(k))}{\partial \vect{w}_r(k)}
%	\right)^\top \vect{x}_{i}} \\
%&\le \frac{\eta \abs{S_{i}^\perp}}{n\sqrt{m}b_{k+1}}  \max_{r \in [m]} \norm{
%	\frac{\partial L_{\xi_k}(\mat{W}(k))}{\partial \vect{w}_r(k)}
%}_2 \\
%&\le  \frac{\eta \abs{S_{i}^\perp}|{u}_{\xi_k}(k)-{y}_{\xi_k}|}{nmb_{k+1}}\\
%&\le  \frac{\eta|{u}_{\xi_k}(k)-{y}_{\xi_k}|}{nb_{k+1}}.
%\end{align*}
%To analyze $I_1^{i}$, by Corollary~\ref{cor:dist_from_init}, we know $\norm{\vect{w}_r(k)-\vect{w}_r(0)} \le R'$ and $\norm{\vect{w}_r(k)-\vect{w}_r(0)} \le R'$ for all $r \in [m]$.
%Furthermore, because $R' < R$, we know $\indict\left\{\vect{w}_r(k+1)^\top \vect{x}_{i}\ge 0\right\}= \indict\left\{\vect{w}_r(k)^\top \vect{x}_{i} \ge 0\right\}$.
%Thus we can find a more convenient expression of $I_1^{i}$ for analysis
%\begin{align*}
%% \xi_{k} is analogue to j in  GD
%I_1^{i}= 
%&-\frac{\eta}{nb_{k+1}}\vect{x}_{\xi_k}^\top \vect{x}_{i}\left(u_{\xi_{k}}(k)-y_{\xi_{k}}\right)\frac{1}{m}\sum_{r \in S_{i}} \indict\left\{\vect{w}_r(k)^\top \vect{x}_{i} \ge 0, \vect{w}_r(k)^\top \vect{x}_{\xi_{k}}\ge 0 \right\}
%\\
%=  &-\frac{\eta}{nb_{k+1}} \left(u_{\xi_{k}}(k)-y_{\xi_{k}}\right)(\mat{H}_{i \xi_{k}}(k) -\mat{H}_{i \xi_{k}}^\perp(k))
%\end{align*} 
%
%Observe from  \eqref{eq:grad_bound} that 
%\begin{align}
%({u_{i}}(k+1)-u_{i}(k))_2^2
%& \le \frac{\eta^2}{b_{k+1}^2}\frac{1}{n^2m}\left(\sum_{r=1}^{m} \norm{\frac{\partial L_{\xi_k}(\mat{W}(k))}{\partial \vect{w}_r(k)}}_2\right)^2 \nonumber\\
%& \le \frac{\eta^2}{b_{k+1}^2}\frac{1}{n^2}\sum_{r=1}^{m} \norm{\frac{\partial L_{\xi_k}(\mat{W}(k))}{\partial \vect{w}_r(k)}}_2^2 \nonumber\\
%&\le   \frac{\eta^2}{b_{k+1}^2}\frac{1}{n^2m}\sum_{r=1}^{m}|y_{\xi_k}-u_{\xi_k}(k)| ^2 \nonumber
%\\
%&\le   \frac{\eta^2}{n^2b_{k+1}^2}|y_{\xi_k}-u_{\xi_k}(k)| ^2 \nonumber 
%\end{align}
%With these estimates at hand, we are ready to prove the induction hypothesis as follows, 
%\begin{align*}
%n\mathbb{E}_{\xi_{k+1}}\left[(y_{\xi_{k+1}}-u_{\xi_{k+1}}(k+1))^2\right]
%= & \| \vy - \vu(k+1)\|^2 \\
%= &  \| \vy - \vu(k)\|^2 +\| \vu(k) - \vu(k+1)\|^2 +2 \sum_{i=1}^n   \left( u_i(k)-u_i(k+1)\right) (y_i-u_i(k))\\
% \leq & \|\vy - \vu(k)\|^2 +   \frac{\eta^2( u_{\xi_k} (k)-y_{\xi_k} )^2}{n b_{k+1}^2}+ 2\sum_{i=1}^n \left( I_2^i+I_1^i\right) (y_i-u_i(k)) \\
%  \leq & \|\vy - \vu(k)\|^2 +    \frac{\eta^2(y_{\xi_k}-u_{\xi_k}(k)) ^2}{nb_{k+1}^2}+ 2 \sum_{i=1}^n |I_2^i||y_i-u_i(k)|\\
%  & +\frac{2\eta \left(u_{\xi_{k}}(k)-y_{\xi_{k}}\right)}{nb_{k+1}}\sum_{i=1}^n(\mat{H}_{i \xi_{k}}^\perp(k)-\mat{H}_{i \xi_{k}}(k))(y_i-u_i(k)) \\
%  \leq & \|\vy - \vu(k)\|^2 +    \frac{\eta^2(y_{\xi_k}-u_{\xi_k}(k)) ^2}{nb_{k+1}^2}+ 2\frac{\eta|{u}_{\xi_k}(k)-{y}_{\xi_k}|}{nb_{k+1}}  \sum_{i=1}^n |y_i-u_i(k)|\\
%  & +\frac{2\eta \left(u_{\xi_{k}}(k)-y_{\xi_{k}}\right)}{nb_{k+1}}\sum_{i=1}^n(\mat{H}_{i \xi_{k}}^\perp(k)-\mat{H}_{i \xi_{k}}(k))(y_i-u_i(k)) \\
%\end{align*} 
% If in probability $b_{k+1}\geq\frac{ n  \eta}{ \lambda_0C}$, we have
% \begin{align*}
%\mathbb{E}_{\xi_1,\cdots,\xi_k}\left[\mathbb{E}_{\xi_{k+1}}\left[(y_{\xi_{k+1}}-u_{\xi_{k+1}}(k+1))^2\right]\right] 
% &\leq\mathbb{E}_{\xi_1,\cdots,\xi_k} \left[\left( 1-\frac{\eta \lambda_0 C }{2 n b_{k+1}} \right)\frac{1}{n}\norm{\vy-\vu(k)}_2^2 \right] \\
%  &\leq \mathbb{E}_{\xi_1,\cdots,\xi_{k}} \left[\left( 1-\frac{\eta \lambda_0 C }{2 n\left( b_{k}+D\right)} \right)\frac{1}{n}\left[\norm{\vy-\vu(k)}_2^2 \right]\right] \\
%   &\leq \mathbb{E}_{\xi_1,\cdots,\xi_{k-1}} \left[\left( 1-\frac{\eta \lambda_0 C }{2 n\left( b_{k}+D\right)} \right)\mathbb{E}_{\xi_{k}}\left[(y_{\xi_{k}}-u_{\xi_{k}}(k))^2\right]\right] 
%\end{align*} 
%where the second inequality due to $b_{k+1}\leq b_k+D$ from assumption 3. 


==> adagrad_stochastic.tex <==
 Note that one should use careful induction to prove the theorem as that in Theorem \ref{thm:main_adagradloss}. We skip these steps, but provide the key step for the derivation of Condition \ref{con:adagrad_sub_stochastic}. We would like to point out the essence of the analysis is how to deal with the correlation between the random variable $b_k$ and loss function $\|\vy-\vu(k)\|$, which is the major difference between the stochastic AdaLoss and deterministic AdaLoss for two-layer neural network. Solving for the correlation between stepsize update $b_t$ and  $\|\vy - \vu(t)\|$ is the major challenges in the proof.  We will first use subsection \ref{sec:condition} to derive the following condition.
 \begin{condition}
	\label{con:adagrad_sub_stochastic} At the $k'$-th iteration,\footnote{For the convenience of induction proof, we define 
		$$ \norm{\vect{y}-\vect{u}(-1)}^2= \norm{\vect{y}-\vect{u}(0)}^2 /\left(1- \frac{\eta  \lambda_0B}{b_{0}}\left(1-\frac{\eta C{\|\vH(0)\|}}{b_{0}} \right) \right). $$
			} we have 
		\begin{align}
& \mathbb{E}_{\xi_{k}}\left[\|\vy-\vu(k+1)\|^2\right] \nonumber\\
\leq& 
% &\leq \left( 1-\frac{2\eta \lambda_0C_1}{b_{k'}} \left(1- \frac{\eta C\|\vH^\infty\|}{2b_{k'}}\right) \right)\mathbb{E}\left[\|\vy-\vu(k'-1)\|^2\right]  
\left(1 -\frac{\eta\lambda_0{B}}{n\sqrt{b_{k}^2+\frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}}}}\left(1
%  +\frac}{ \sqrt{b_{k}^2+\alpha^2\frac{ \|\vy-\vu(k)\|^2}{\sqrt{ n}}} }
 -\frac{ n(2\alpha n^{-\frac{3}{4}} +\eta)}{ \eta \lambda_0B\sqrt{b_{k}^2+\frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}}} } \right)\right)\|\vy-\vu(k)\|^2 \nonumber
\end{align}
 where $B = 1-\frac{ 2nC_2(\sqrt{n}+n)R}{\lambda_0\delta} = \Theta(1)$ for $R=\frac{c\lambda_0\delta}{n^3}$.
 \end{condition}
 
Now that we have the condition, we can prove the following lemmas for the convergence. We will give the proof for Lemma \ref{lem:adagrad_stochastic1} in subsection \ref{sec:proof1}, and the proof for Lemma \ref{lem:adagrad_stochastic2} in subsection \ref{sec:proof2}. Finally, we have Lemma \ref{lem:adagrad_stochastic3}, which is directly from Lemma \ref{highp}.

%  \begin{lem}
% \label{lem:adagrad_stochastic0}
% Let $T_0\geq 1$ be the first index such that $b_{T_0+1} \geq \frac{2n(2\alpha n^{-\frac{3}{4}}+\eta)}{ \lambda_0 B}$ from $b_{T_0} < \frac{2n(2\alpha n^{-\frac{3}{4}}+\eta)}{ \lambda_0 B} $. Suppose Condition \ref{con:adagrad_sub} holds for $k'=0,1,\ldots,k$. Then
% \begin{align*}
% \norm{\vy-\vu(T_0)}^2
%  \leq & \norm{\vy-\vu(0)}^2 +  \frac{\eta(2\alpha n^{-\frac{3}{4}} +\eta)\sqrt{n}}{\alpha^2} \log \left( \frac{2n(2\alpha n^{-\frac{3}{4}}+\eta)}{\eta \lambda_0 B b_0} \right).
% \end{align*}
% \end{lem}
\begin{lem}
\label{lem:adagrad_stochastic1}
Suppose Condition~\ref{con:adagrad_sub_stochastic} holds for $k'=0,\ldots,k$ and   $ b_k$  is updated by Stochastic AdaLoss. Let $T_0\geq 1$ be the first index such that $b_{T_0}\geq \frac{2n(2\alpha n^{-\frac{3}{4}}+\eta)}{ \lambda_0 B} $.  Then for every $r \in [m]$ and $k = 0,1,\cdots$, with high probability, $1-\delta'$
\begin{align*}
 & b_{k}\leq \frac{1}{\delta'} \left(b_{T_0} + \frac{2\alpha^2 \sqrt{n}}{\eta {\lambda_0}B}\mathbb{E}\left[ \norm{\vy-\vu(T_0)}^2\right] + \sqrt{  \frac{\alpha^2 \mathbb{E}\left[ \|\vy-\vu(T_0)\|^2\right]}{\sqrt{ n}}}\right) ;\\
&\mathbb{E}\left[\|\vw_r(k+T_0)-\vw_r(T_0)\| \right]
\leq \frac{4\sqrt{n}}{ {\lambda_0 }B\sqrt{m}}\mathbb{E}\left[ \norm{\vy-\vu(T_0)}\right].
\end{align*}
\end{lem} 
 \begin{lem}
\label{lem:adagrad_stochastic2}
Let $T_0\geq 1$ be the first index such that $b_{T_0+1} \geq \frac{2n(2\alpha n^{-\frac{3}{4}}+\eta)}{ \lambda_0 B}$ from $b_{T_0} < \frac{2n(2\alpha n^{-\frac{3}{4}}+\eta)}{ \lambda_0 B} $. Suppose Condition \ref{con:adagrad_sub} holds for $k'=0,1,\ldots,k$. Then,
\begin{align*}
\mathbb{E}\left[\norm{\vy-\vu(T_0)}^2\right]
 \leq & \mathbb{E}\left[\norm{\vy-\vu(0)}^2\right] + \left(\frac{\eta^2\sqrt{n}}{\alpha^2}+\frac{2\eta n^{-\frac{3}{4}}}{\alpha}\right)\log \left( \frac{2n(2\alpha n^{-\frac{3}{4}}+\eta)}{\eta \lambda_0 B b_0} \right).
\end{align*}
\end{lem}
\begin{lem}
\label{lem:adagrad_stochastic3} 
Under the same hypothesis as Lemma \ref{lem:adagrad_stochastic2} and Assumption \ref{ruil}. Suppose we start with small initialization: $0<b_0< \frac{2n(2\alpha n^{-\frac{3}{4}}+\eta)}{ \lambda_0 B}$.  Then with probability $1- \exp(-\frac{\|\Delta\|^2}{2(N\gamma(1-\gamma)+\delta)})$, after 
\begin{align*}
\hat{T} =  \left\lceil \frac{1}{\lambda_0\gamma\varepsilon} \left(\left(\frac{2n(2\alpha n^{-\frac{3}{4}}+\eta)}{ \lambda_0 B}\right)^2 -b_0^2\right)+\frac{\delta}{\gamma} +1  \right\rceil,
\end{align*}
 either  $b_{\hat{T}+1}\geq \frac{2n(2\alpha n^{-\frac{3}{4}}+\eta)}{ \lambda_0 B}$ or  $\min_{t\in [\hat{T}]}\|\vy-\vu(t)\|^2\leq \varepsilon.$
\end{lem}

\subsection{Derivation of Condition \ref{con:adagrad_sub_stochastic} }\label{sec:condition}

 Note first that the stepsize in \eqref{eq:defineQQ} need to be replaced by $\eta/ b_{k+1}$, i.e.,
\begin{align}
[\vu(k+1)]_i - [\vu(k)]_i
= & \frac{1}{\sqrt{m}}\sum_{r=1}^{m} a_r \left(\relu{\left(
	\vect{w}_r(k) - \frac{\eta}{b_{k+1}}\frac{\partial L_{\xi_k}(\mat{W}(k))}{\partial \vect{w}_r(k)}
	\right)^\top \vect{x}_i} - \relu{\vect{w}_r(k)^\top \vect{x}_i}\right) \nonumber\\
	=& \frac{\eta}{b_{k+1}} \left( [\vQ({\xi_k})]_i+[\widetilde{\vQ}({\xi_k})]_i \right)
	\label{eq:defineQQ_ada}
\end{align}
For expectation inequality \eqref{eq:y-u1}, we replace $\eta$ with $\frac{\eta}{b_k}$,
\begin{align*}
&\mathbb{E}_{\xi_k}\left[ \| \vy - \vu(k+1)\|^2\right] \\
= & \norm{\vect{y}-\vect{u}(k)}_2^2+ \mathbb{E}_{\xi_{k}}\left[\norm{\vect{u}(k+1)-\vect{u}(k)}_2^2\right] - 2 \left(\vect{y}-\vect{u}(k)\right)^\top \mathbb{E}_{\xi_{k}}\left[\left(\vect{u}(k+1)-\vect{u}(k)\right) \right]\nonumber
%\\
%= & \|\vy - \vu(k)\|^2 + \mathbb{E}_{\xi_k}\left[ \| \vu(k) - \vu(k+1)\|^2\right] +  2\eta \bigg\langle{ \mathbb{E}_{\xi_k}\left[ \frac{\widetilde{ \mat{Q}}_2(\xi_k)}{b_{k+1}} \right], \vy-\vu(k) \bigg\rangle} \\
%& +  \mathbb{E}_{\xi_k}\left[\frac{2\eta \left(y_{\xi_{k}}-u_{\xi_{k}}(k)\right)}{nb_{k+1}} \sum_{i=1}^n
%\left(\mat{H}_{i \xi_{k}}^\perp(k) -\mat{H}_{i \xi_{k}}(k)\right)(y_i-u_i(k))\right]
\end{align*} 
We estimate $ \mathbb{E}_{\xi_{k}}\left[\norm{\vect{u}(k+1)-\vect{u}(k)}_2^2\right]$  and $\mathbb{E}_{\xi_{k}}\left[\left(\vect{u}(k+1)-\vect{u}(k)\right) \right]$ and in subsection \ref{sec:var} and \ref{sec:mean} respectively. 
\subsubsection{Variance $\mathbb{E}_{\xi_{k}}\left[\norm{\vect{u}(k+1)-\vect{u}(k)}_2^2\right]$ } \label{sec:var}
Observe from  \eqref{eq:defineUU} that 
\begin{align}
\mathbb{E}_{\xi_k}\left[\norm{\vect{u}(k+1)-\vect{u}(k)}_2^2\right]
%&= \sum_{i=1}^n\mathbb{E}_{\xi_k}\left[\left(u_i(k+1)-u_i (k) \right)^2\right] \nonumber\\
&\leq \eta^2 \sum_{i=1}^n\mathbb{E}_{\xi_k}\left[\sum_{r=1}^m\abs{ \frac{1}{b_{k+1}}\bigg \langle{ \frac{\partial L_{\xi_k}(\mat{W}(k))}{\partial \vect{w}_r(k)}, \vx_i \bigg\rangle}}^2 \right]\nonumber\\
&\leq  \eta ^2   \sum_{i=1}^n \mathbb{E}_{\xi_k}\left[  \frac{|y_{\xi_k}-u_{\xi_k}(k)|^2}{{b_k^2+\alpha^2\sqrt{n} {|y_{\xi_k}-u_{\xi_k}(k)|^2 }} }\right]\nonumber\\
&\leq    \frac{ \eta^2n \mathbb{E}_{\xi_k}\left[|y_{\xi_k}-u_{\xi_k}(k)|^2\right]}{{b_k^2+\alpha^2 \sqrt{n}{ \mathbb{E}_{\xi_k}\left[|y_{\xi_k}-u_{\xi_k}(k)|^2\right] }} }\nonumber\\
&=  \frac{  \eta^2 \norm{\vect{y}-\vect{u}(k)}_2^2 }{{b_k^2+ \alpha^2 \norm{\vect{y}-\vect{u}(k)}^2/\sqrt{n} }}.
\end{align}
where at the third step we apply Jensen's inequality to the concave function $f(x)=\frac{x}{a+bx}, \forall a>0,b>0 $.

\subsubsection{Mean $\mathbb{E}_{\xi_{k}}\left[\vect{u}(k+1)-\vect{u}(k)\right]$} \label{sec:mean}
First, note that
\begin{align}
  & - \frac{1}{2\eta}\bigg\langle{ \vect{y}-\vect{u}(k), \mathbb{E}_{\xi_{k}}\left[\left(\vect{u}(k+1)-\vect{u}(k)\right) \right]  \bigg\rangle} \nonumber\\
  =&-\bigg\langle{ \mathbb{E}_{\xi_k}\left[ \frac{\widetilde{ \mat{Q}}(\xi_k)}{b_{k+1}} \right], \vy-\vu(k) \bigg\rangle} 
+ \sum_{i=1}^n(y_i-u_i(k)) \mathbb{E}_{\xi_k}\left[\frac{ \left(y_{\xi_{k}}-u_{\xi_{k}}(k)\right)\left(\mat{H}_{i \xi_{k}}^\perp(k) -\mat{H}_{i \xi_{k}}(k)\right)}{b_{k+1}} 
\right]  \nonumber\\
\leq& \| \vy-\vu(k) \| \bigg\|\mathbb{E}_{\xi_k}\left[ \frac{\widetilde{ \mat{Q}}(\xi_k)}{b_{k+1}} \right]\bigg\|
+ \underbrace{\sum_{i=1}^n (y_i-u_i(k)) \mathbb{E}_{\xi_k}\left[ \left(  \frac{ \left(y_{\xi_{k}}-u_{\xi_{k}}(k)\right)
\mat{H}_{i \xi_{k}} }{ \sqrt{ b_{k}^2+ \alpha^2 \frac{\|\vy-\vu(k)\|}{\sqrt{n}} }} -\frac{ \left(y_{\xi_{k}}-u_{\xi_{k}}(k)\right)
\mat{H}_{i \xi_{k}} }{b_{k+1}}\right) \right]}_{term1} \nonumber\\
&- \underbrace{ \sum_{i=1}^n(y_i-u_i(k))  \frac{\mathbb{E}_{\xi_k}\left[ \left(y_{\xi_{k}}-u_{\xi_{k}}(k)\right)
\mat{H}_{i \xi_{k}}\right]}{ \sqrt{ b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }} }_{term2}
 +  \underbrace{\sum_{i=1}^n(y_i-u_i(k)) \mathbb{E}_{\xi_k}\left[\frac{ \left(y_{\xi_{k}}-u_{\xi_{k}}(k)\right)\mat{H}_{i \xi_{k}}^\perp(k)}{b_{k+1}} 
\right]}_{term3}  \label{eq:innerPro}
\end{align}
We first upper bound  the expectation of $term3$ as follows
\begin{align*}
 \mathbb{E}_{\xi_k}\left[\frac{ \left(y_{\xi_{k}}-u_{\xi_{k}}(k)\right)
\mat{H}_{i \xi_{k}}^\perp(k)}{b_{k+1}} \right]  
&\leq  \sqrt{  \mathbb{E}_{\xi_k}\left[ \frac{ \left(y_{\xi_{k}}-u_{\xi_{k}}(k)\right)^2}{b_{k+1}^2} \right] }\sqrt{ \mathbb{E}_{\xi_k}\left[ 
\left(\mat{H}_{i \xi_{k}}^\perp(k) \right)^2  \right] } \\
&\leq  \frac{\norm{\vect{y}-\vect{u}(k)}/\sqrt{n} }{{ \sqrt{b_k^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }}} \frac{\sum_{j=1}^n\abs{\mat{H}_{i j}^\perp(k)}}{\sqrt{n}} \\
&\leq  \frac{\norm{\vect{y}-\vect{u}(k)}}{{ \sqrt{b_k^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }}} \frac{\abs{S_i^\perp} }{m}
\end{align*}
by recalling that $
\mat{H}_{ij}^\perp(k) = \frac{1}{m}\sum_{r \in S_i^\perp}\vect{x}_i^\top \vect{x}_j \indict\left\{\vect{w}_r(k)^\top \vect{x}_i \ge 0, \vect{w}_r(k)^\top \vect{x}_j \ge 0\right\}
$. Thus $term3$ reduces to 
\begin{align*}
term3 &\leq   \frac{\norm{\vect{y}-\vect{u}(k)}}{{ \sqrt{b_k^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }}} \frac{\sum_{i=1}^n|y_i-u_i(k)|\abs{S_i^\perp}}{m}\\
 &\leq  \frac{\norm{\vect{y}-\vect{u}(k)}}{{ \sqrt{b_k^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }}} \frac{ \sqrt{ \sum_{i=1}^n|y_i-u_i(k)|^2} \sqrt{ \sum_{i=1}^n\abs{S_i^\perp}^2 }}{m} \\
  &\leq  \frac{ \norm{\vect{y}-\vect{u}(k)}^2 C_2\sqrt{n}R/\delta}{ \sqrt{b_k^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }}
\end{align*}
For $term2$, we immediately have that 
\begin{align*}
 \sum_{i=1}^n(y_i-u_i(k))  \frac{\mathbb{E}_{\xi_k}\left[ \left(y_{\xi_{k}}-u_{\xi_{k}}(k)\right)
\mat{H}_{i \xi_{k}}\right]}{ \sqrt{ b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }} 
&= \frac{ \left( \vy-\vu(k)\right)^\top\mat{H} \left(\vy-\vu(k) \right)  }{ n\sqrt{ b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }}
\geq \frac{\lambda_0 \| \vy-\vu(k)\|^2}{  2n\sqrt{ b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }} 
\end{align*}
For $term1$, as we observe that 
\begin{align*}
  \abs{\frac{1}{ \sqrt{ b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }} -\frac{1}{b_{k+1}}}
  &=\frac{ \abs{ \alpha n^{1/4} |y_{\xi_k}-x_{\xi_k}|-  \alpha \frac{ \|\vy-\vu(k)\|}{n^{1/4}}}\abs{ \alpha n^{1/4} |y_{\xi_k}-x_{\xi_k}|+ \alpha \frac{ \|\vy-\vu(k)\|}{n^{1/4}}}}{ b_{k+1}\sqrt{ b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} } \left( b_{k+1}+ \sqrt{ b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }  \right)  } \\
&\leq \frac{ \alpha n^{1/4} \abs{  |y_{\xi_k}-x_{\xi_k}| - \frac{ \|\vy-\vu(k)\|}{ \sqrt{n} }}}{ b_{k+1}\sqrt{ b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }} 
%   \\
%     &\leq\frac{ \alpha^2 \sqrt{n} |y_{\xi_k}-x_{\xi_k}| - \alpha^2 \|\vy-\vu(k)\|/\sqrt{n}}{ b_{k+1}\sqrt{ b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} } \left( b_{k+1}+ \sqrt{ b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }  \right)  }
\end{align*}
which thus gives
\begin{align} 
&\mathbb{E}_{\xi_k}\left[ \left(  \frac{ \left(y_{\xi_{k}}-u_{\xi_{k}}(k)\right)
\mat{H}_{i \xi_{k}} }{ \sqrt{ b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }} -\frac{ \left(y_{\xi_{k}}-u_{\xi_{k}}(k)\right)
\mat{H}_{i \xi_{k}} }{b_{k+1}}\right) \right] \nonumber\\ 
%equation1 
\leq  & \mathbb{E}_{\xi_k}\left[ \frac{\alpha n^{1/4} | (y_{\xi_{k}}-u_{\xi_{k}}(k))
\mat{H}_{i \xi_{k}} | \left(|y_{\xi_k}-x_{\xi_k}| + \frac{\|\vy-\vu(k)\|  }{\sqrt{n}}  \right)}  { b_{k+1}\sqrt{ b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} } }\right] \nonumber\\ 
%equation2
 \leq & \frac{\alpha n^{1/4} }{ \sqrt{ b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }}\mathbb{E}_{\xi_k}\left[ \frac{  |y_{\xi_{k}}-u_{\xi_{k}}(k)|^2}{b_{k+1}}
+ \frac{ |y_{\xi_{k}}-u_{\xi_{k}}(k)| \|\vy-\vu(k)\|^2 }{ \sqrt{n} b_{k+1}  }\right] \nonumber\\ 
%equation3
 \leq & \frac{\alpha n^{1/4} }{ \sqrt{ b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }} \left(
%  \frac{ \mathbb{E}_{\xi_k}\left[ |y_{\xi_{k}}-u_{\xi_{k}}(k)|^2 \right]}{\sqrt{b_{k}^2+\alpha^2\sqrt{ n}  \mathbb{E}_{\xi_k}\left[ |y_{\xi_{k}}-u_{\xi_{k}}(k)|^2 \right]}}
% + 
\frac{ \mathbb{E}_{\xi_k}\left[ |y_{\xi_{k}}-u_{\xi_{k}}(k)|^2 \right]+\sqrt{\mathbb{E}_{\xi_k}\left[ |y_{\xi_{k}}-u_{\xi_{k}}(k)|^2 \right] }\frac{ \|\vy-\vu(k)\|}{\sqrt{n}} }{  \sqrt{ b_{k}^2+\alpha^2\sqrt{ n} \mathbb{E}_{\xi_k}\left[ |y_{\xi_{k}}-u_{\xi_{k}}(k)|^2 \right]} } \right)\nonumber\\ 
%equation4
= & \frac{2\alpha \|\vy-\vu(k)\|^2/n^{3/4} }{  b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }
\end{align}
Finally, we estimate the expectation of $ \frac{[\widetilde{\vQ}({\xi_k})]_i}{b_{k+1}}$,
\begin{align}
\mathbb{E}_{\xi_k}\left[ \frac{[\widetilde{\vQ}({\xi_k})]_i}{b_{k+1}} \right]
&\le  \frac{  |S_{i}^\perp|}{ {m}} \mathbb{E}_{\xi_k}\left[  \frac{|y_{\xi_k}-u_{\xi_k}(k)|^2 }{\sqrt{b_{k+1}^2 + \alpha^2 \sqrt{n} |y_{\xi_k}-u_{\xi_k}(k)|}}\right] \\
 & \leq   \frac{  |S_{i}^\perp|}{  {m}}  \frac{ \sqrt{ \mathbb{E}_{\xi_k}\left[ |y_{\xi_k}-u_{\xi_k}(k)|^2 \right] } }{ \sqrt{b_{k}^2 + \alpha^2 \sqrt{n}{ \mathbb{E}_{\xi_k}\left[ |y_{\xi_k}-u_{\xi_k}(k)|^2 \right] } }} \nonumber\\
  &= \frac{  |S_{i}^\perp|}{ m} \frac{ \|\vy-\vu(k)\|}{ \sqrt{b_{k}^2+\alpha^2 \|\vy-\vu(k)\|^2/\sqrt{ n}}}\nonumber
\end{align}
where we apply Jensen's inequality to the concave function $y=\frac{\sqrt{x}}{{\sqrt{a+b{x}}}}$  for any $a>0,b>0$.
 By Lemma \ref{lem:bounds_Si_perp}, we have $ \sum_{i=1}^n |S_{i}^\perp| \leq \frac{C_2mnR}{\delta}$
\begin{align*}
\bigg\|\mathbb{E}_{\xi_k}\left[ \frac{\widetilde{ \mat{Q}}(\xi_k)}{b_{k+1}} \right]\bigg\| \leq \sum _{i=1}^n  \abs{ \mathbb{E}_{\xi_k}\left[ \frac{[\widetilde{\vQ}({\xi_k})]_i}{b_{k+1}} \right]} 
&\leq \frac{ \|\vy-\vu(k)\|  \sum_{i=1}^n |S_{i}^\perp| }{  m\sqrt{n} \sqrt{b_{k}^2+\alpha^2 \|\vy-\vu(k)\|^2/\sqrt{ n}}} \\
&= \frac{  C_2\sqrt{n}R\|\vy-\vu(k)\|/\delta}{ \sqrt{b_{k}^2+\alpha^2 \|\vy-\vu(k)\|^2/\sqrt{ n}}} 
\end{align*}
With above bound for $\bigg\|\mathbb{E}_{\xi_k}\left[ \frac{\widetilde{ \mat{Q}}(\xi_k)}{b_{k+1}} \right]\bigg\|$,  the upper bound of $term1$, $term3$ and the lower bound for $term2$, the 
inequality \eqref{eq:innerPro} reduce to 
\begin{align*}
  & - \frac{1}{2\eta}\bigg\langle{ \vect{y}-\vect{u}(k), \mathbb{E}_{\xi_{k}}\left[\left(\vect{u}(k+1)-\vect{u}(k)\right) \right]  \bigg\rangle} \nonumber\\
\leq & \frac{ \|\vy-\vu(k)\|^2 C_2\sqrt{n}R/\delta}{ \sqrt{b_{k}^2+\alpha^2 \frac{\|\vy-\vu(k)\|^2}{\sqrt{ n}}}} + \frac{2\alpha n^{-3/4} \|\vy-\vu(k)\|^2 }{ b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}}} -\frac{\lambda_0 \| \vy-\vu(k)\|^2}{  2n\sqrt{ b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }}+ \frac{C_2nR \norm{\vect{y}-\vect{u}(k)}^2}{ \delta\sqrt{b_k^2+ \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{n}} }}\\
= & \left( \frac{ C_2(\sqrt{n}+n)R}{\delta}  +\frac{2\alpha n^{-3/4} }{ \sqrt{b_{k}^2+\alpha^2\frac{ \|\vy-\vu(k)\|^2}{\sqrt{ n}}} } -\frac{\lambda_0}{2n} \right)  \frac{ \|\vy-\vu(k)\|^2 }{ \sqrt{b_{k}^2+\alpha\frac{\|\vy-\vu(k)\|^2}{\sqrt{ n} }}} 
\end{align*}
Bringing the two terms  $\bigg\langle{ \vect{y}-\vect{u}(k), \mathbb{E}_{\xi_{k}}\left[\left(\vect{u}(k+1)-\vect{u}(k)\right) \right]  \bigg\rangle}$ and $ \mathbb{E}_{\xi_{k}}\left[\norm{\vect{u}(k+1)-\vect{u}(k)}_2^2\right]$ from subsection \ref{sec:var} and \ref{sec:var},  we have
\begin{align}
&\mathbb{E}_{\xi_{k}}\left[\norm{\vect{y}-\vect{u}(k+1)}^2 \right] -\norm{\vect{y}-\vect{u}(k)}^2  \nonumber\\
 \le &\left(-\frac{\lambda_0}{2n}+\frac{ C_2(\sqrt{n}+n)R}{\delta} 
%  +\frac}{ \sqrt{b_{k}^2+\alpha^2\frac{ \|\vy-\vu(k)\|^2}{\sqrt{ n}}} }
 + \frac{2\alpha n^{-3/4} +\eta}{ \sqrt{b_{k}^2+\frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}}} } \right)  \frac{ 2\eta \|\vy-\vu(k)\|^2}{ \sqrt{b_{k}^2+\frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}}} }   \nonumber\\
= & -\frac{\eta\lambda_0{B}}{n\sqrt{b_{k}^2+\frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}}}}\left(1
%  +\frac}{ \sqrt{b_{k}^2+\alpha^2\frac{ \|\vy-\vu(k)\|^2}{\sqrt{ n}}} }
 -\frac{ n(2\alpha n^{-3/4} +\eta)}{ \lambda_0B\sqrt{b_{k}^2+\frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}}} } \right) \|\vy-\vu(k)\|^2   \label{eq:adaloss-stoch}
%  \\
% \leq & - \left( 1- \frac{2n}{\lambda_0} \left( \frac{2 C_2\sqrt{n}R}{\delta}+ \frac{ \alpha^2 +\eta \sqrt{b_{k}^2+ \frac{\alpha^2 \|\vy-\vu(k)\|}{\sqrt{ n}}}}{b_{k}^2+\frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}} } \right)  \right)\frac{ \lambda_0\eta \|\vy-\vu(k)\|^2}{n \sqrt{b_{k}^2+\frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}}} } 
\end{align}
where $B = 1-\frac{ 2nC_2(\sqrt{n}+n)R}{\lambda_0\delta} = \Theta(1)$ for $R=\frac{c\lambda_0\delta}{n^3}$.
\subsection{Proof for the Lemmas \ref{lem:adagrad_stochastic1}}\label{sec:proof1}
\begin{proof}
%  we have
% \begin{align*}
% \frac{\lambda_0}{2n}-\frac{ C_2(\sqrt{n}+n)R}{\delta} 
% %  +\frac}{ \sqrt{b_{k}^2+\alpha^2\frac{ \|\vy-\vu(k)\|^2}{\sqrt{ n}}} }
% &\geq \frac{2\alpha n^{-\frac{3}{4}} +\eta}{ \sqrt{b_{k}^2+\frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}}} },
% \end{align*}
% and 
For Condition \ref{con:adagrad_sub_stochastic}, we   immediately have the contraction
\begin{align}
&\mathbb{E}_{\xi_{k}}\left[\norm{\vect{y}-\vect{u}(k+1)}^2 \right]  
 \le \left(1-\frac{ \eta \lambda_0B}{2n \sqrt{b_{k}^2+\frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}}} }  \right)  \|\vy-\vu(k)\|^2 \label{eq:key-contraction}
%  \\
%  \Rightarrow \quad &\mathbb{E}_{\xi_{k}}\left[\norm{\vect{y}-\vect{u}(k+1)} \right]  
%  \le \left(1-\frac{ \eta \lambda_0}{4n \sqrt{b_{k}^2+\frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}}} }  \right)  \|\vy-\vu(k)\|
\end{align}
since 
 \begin{align}
    b_{k}\geq \frac{2n(2\alpha n^{-\frac{3}{4}}+\eta)}{\lambda_0 B} \quad \Rightarrow \quad 1
%  +\frac}{ \sqrt{b_{k}^2+\alpha^2\frac{ \|\vy-\vu(k)\|^2}{\sqrt{ n}}} }
 -\frac{ n(2\alpha n^{-\frac{3}{4}} +\eta)}{  \lambda_0B\sqrt{b_{k}^2+\frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}}} } \geq \frac{1}{2}\label{eq:b-stochastic}
 \end{align}
 
Taking the expectation of the above inequality for both sides,
\begin{align}
&\mathbb{E}\left[\norm{\vect{y}-\vect{u}(k+1)}^2 \right]  
 \le  \mathbb{E}\left[\norm{\vect{y}-\vect{u}(k)}^2 \right]- \mathbb{E}\left[ \frac{ \eta \lambda_0 B  \|\vy-\vu(k)\|^2}{2n \sqrt{b_{k}^2+\frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}}} }\right] \label{eq:keycontraction1}
\end{align}
% Suppose we have the first iteration index $T_0$ such that $b_{T_0+1}\geq \frac{2n(2\alpha n^{-\frac{3}{4}}+\eta)}{ \lambda_0 B} $ and $b_{T_0}\leq \frac{2n(2\alpha n^{-\frac{3}{4}}+\eta)}{ \lambda_0 B} $, then we have contraction like \eqref{eq:keycontraction1}. 
Telescoping sum for $k=T_0,T_0+1,\ldots,T$ gives
\begin{align}
\mathbb{E}\left[  \sum_{k=T_0}^T\frac{ \eta \lambda_0 B  \|\vy-\vu(k)\|^2 }{2n \sqrt{b_{k}^2+\frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}}} }\right] \leq   \norm{\vect{y}-\vect{u}(T_0)}^2 
%-\mathbb{E}\left[\norm{\vect{y}-\vect{u}(T+1)} \right]  
\end{align}
Observe that by Jensen inequality, we have $\mathbb{E}\left[ b_{k+1} \right], T_0\leq k\leq T$ bounded by
\begin{align*}
\mathbb{E}\left[ b_{k+1} \right] &\leq   \mathbb{E}\left[b_{k} \right] + \mathbb{E}\left[\frac{\alpha^2\sqrt{n}|y_{\xi_{k}} - u_{\xi_{k}} (k)|^2 }{b_{k+1}}  \right] \\
&\leq  \mathbb{E}\left[b_{k} \right] + \mathbb{E}\left[\frac{\alpha^2\sqrt{n}\mathbb{E}_{\xi_k}\left[ |y_{\xi_{k}} - u_{\xi_{k}} (k)|^2\right]}{ \sqrt{ b_{k}^2 +\alpha^2\sqrt{n}\mathbb{E}_{\xi_k}\left[ |y_{\xi_{k}} - u_{\xi_{k}} (k)|^2\right] }}  \right] \\
&=  \mathbb{E}\left[b_{k} \right] + \mathbb{E}\left[\frac{\alpha^2 \frac{ \|\vy-\vu(k)\|^2}{\sqrt{n}}}{ \sqrt{ b_{k}^2 +\alpha^2\frac{ \|\vy-\vu(k)\|^2}{\sqrt{n}}} } \right] \\
&\leq  b_{T_0}  + \mathbb{E}\left[\sum_{t=T_0}^{k}\frac{\alpha^2 \frac{ \|\vy-\vu(k)\|^2}{\sqrt{n}}}{ \sqrt{ b_{t}^2 +\alpha^2\frac{ \|\vy-\vu(k)\|^2}{\sqrt{n}}} } \right] \\
&\leq  b_{T_0} + \frac{2\alpha^2 \sqrt{n}}{\eta {\lambda_0}B}\mathbb{E}\left[ \norm{\vy-\vu(T_0)}^2\right].
%\\
%\Rightarrow \quad   \mathbb{E}&\left[ b_{k+1} +\alpha^2\sqrt{ n} \|\vy-\vu(k+1)\|  \right] \leq   b_{0} + \frac{2\alpha n^{-\frac{3}{4}} n^{3/2}}{\eta {\lambda_0}C_1} \norm{\vy-\vu(0)} 
%- \mathbb{E}\left[\norm{\vect{y}-\vect{u}(k+1)} \right]  \right) 
\end{align*}
Also note from  inequality \eqref{eq:keycontraction1}, that $\mathbb{E}\left[\norm{\vect{y}-\vect{u}(k+1)} \right] \leq \norm{\vy-\vu(T_0)} $.  Thus, for $k>T_0$,
\begin{align*}
\mathbb{E}\left[ \sqrt{b_{k}^2 +  \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}}}\right]
&\leq \mathbb{E}\left[ b_{k} \right]+ \sqrt{  \frac{\alpha^2 \mathbb{E}\left[ \|\vy-\vu(k)\|^2\right]}{\sqrt{ n}}} \\
&\leq  \underbrace{b_{T_0} + \frac{2\alpha^2 \sqrt{n}}{\eta {\lambda_0}B}\mathbb{E}\left[ \norm{\vy-\vu(T_0)}^2\right] + \sqrt{  \frac{\alpha^2 \mathbb{E}\left[ \|\vy-\vu(T_0)\|^2\right]}{\sqrt{ n}}}}_{\mathcal{Q}_{T_0}}\\
\Rightarrow \sqrt{b_{k}^2 +  \frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}}} &\leq  \frac{\mathcal{Q}_{T_0}}{\delta'}  \quad \text{with high probability} \quad 1-\delta'
\end{align*}
%  Then, with probability $1-\delta'$, $\forall k \leq T$
% \begin{align}
%  \sqrt{b_{k}^2+\frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}}}\leq b_{k+1} + \sqrt{ \alpha^2\sqrt{ n} \|\vy-\vu(k+1)\|} \leq \frac{b_{\infty} }{\delta'}.
% \end{align}

As for the  upper bound of $\|\vw_r(k)-\vw_r(T_0)\|$ for $t>T_0$ we repeat \eqref{eq:key-contraction} but without square. That is,
\begin{align*}
\mathbb{E}\left[\norm{\vect{y}-\vect{u}(k+1)} \right]  
 &\le \sqrt{\mathbb{E}\left[\norm{\vect{y}-\vect{u}(k+1)}^2 \right]} \\
 &\le \mathbb{E}\left[\left(1-\frac{ \eta \lambda_0B}{4n \sqrt{b_{k}^2+\frac{\alpha^2 \|\vy-\vu(k)\|^2}{\sqrt{ n}}} }  \right)  \|\vy-\vu(k)\| \right] \nonumber\\
 & \leq \mathbb{E}\left[\norm{\vy-\vu(T_0)} \right] -\sum_{\ell=T_0}^{k}\mathbb{E}\left[ \frac{ \eta \lambda_0 B  \|\vy-\vu(\ell)\|}{4n \sqrt{b_{\ell}^2+\frac{\alpha^2 \|\vy-\vu(\ell)\|^2}{\sqrt{ n}}} }\right] \label{eq:keycontraction1} \\
 \Rightarrow \quad \quad  \sum_{\ell=T_0}^{k}\mathbb{E}&\left[ \frac{ \eta \lambda_0 B  \|\vy-\vu(\ell)\|}{4n \sqrt{b_{\ell}^2+\frac{\alpha^2 \|\vy-\vu(\ell)\|^2}{\sqrt{ n}}} }\right] \leq\mathbb{E}\left[\norm{\vy-\vu(T_0)} \right].
 \end{align*}
Thus we have for $k\geq T_0$
\begin{align*}
\mathbb{E}\left[ \|\vw_r(k+1)-\vw_r(T_0)\| \right]
\leq& \sum_{t=T_0}^{k} \mathbb{E}\left[ \frac{\eta }{b_{t+1}} \| \frac{\partial L_{\xi_t}(\vW{(t)})}{\partial \vw_r } \|\right] \\
% \leq& \sum_{t=T_0}^{k} \mathbb{E}\left[\frac{\eta \mathbb{E}_{\xi_k}\left[ \frac{\partial L_{\xi_t}(\vW{(t)})}{\partial \vw_r } \right]}{ \sqrt{ b_{t}^2 +\alpha^2\sqrt{n}\mathbb{E}_{\xi_t}\left[ |y_{\xi_{t}} - u_{\xi_{t}} (t)|^2\right] }}  \right] \\
\leq &\mathbb{E}\left[\sum_{t=0}^{k}\frac{\eta\frac{ \|\vy-\vu(k)\|}{\sqrt{nm}}}{ \sqrt{ b_{t}^2 +\alpha^2\frac{ \|\vy-\vu(t)\|^2}{\sqrt{n}}} } \right] \\
%&\leq  b_{0}  + \mathbb{E}\left[\sum_{t=0}^{T}\frac{\alpha^2 \frac{ \|\vy-\vu(k)\|^2}{\sqrt{n}}}{ \sqrt{ b_{t}^2 +\alpha^2\frac{ \|\vy-\vu(k)\|^2}{\sqrt{n}}} } \right] \\
\leq &\frac{4\sqrt{n}}{ {\lambda_0 }B\sqrt{m}}\mathbb{E}\left[ \norm{\vy-\vu(T_0)}\right].
%\leq & \frac{\eta \sqrt{n}}{\sqrt{m}}\sum_{t=0}^{k}\frac{1}{b_{t+T_0}} \| \vy - \vu(t+T_0-1)\| \\
\end{align*}
where the second inequality is due to \eqref{eq:sgd_grad_bound}.
\end{proof}
\subsection{Proof of Lemma \ref{lem:adagrad_stochastic2}}\label{sec:proof2}
By Condition \ref{con:adagrad_sub_stochastic}, if $b_{t} \leq \frac{2n(2\alpha n^{-\frac{3}{4}}+\eta)}{ \lambda_0 B},$
\begin{align}
\mathbb{E}\left[\norm{\vy-\vu(T_0)}^2 \right] &\leq  \mathbb{E}\left[ \norm{\vy-\vu(T_0-1)}^2\right]+(2\alpha n^{-\frac{3}{4}} +\eta)\eta \mathbb{E}\left[\frac{\norm{\vy-\vu(T_0-1)}^2}{ {b_{T_0-1}^2+\frac{\alpha^2 \|\vy-\vu(T_0-1)\|^2}{\sqrt{ n}}} }\right]\nonumber\\
    &\leq\mathbb{E}\left[\norm{\vy-\vu(0)}^2\right] + \frac{\eta(2\alpha n^{-\frac{3}{4}} +\eta)\sqrt{n}}{\alpha^2}\sum_{t=0}^{T_0-1} \mathbb{E}\left[\frac{ \alpha^2\norm{\vy-\vu(t)}^2/\sqrt{n}}{ {b_{t}^2+\frac{\alpha^2 \|\vy-\vu(t)\|^2}{\sqrt{ n}}} }\right]  \nonumber \\
        &\leq \mathbb{E}\left[\norm{\vy-\vu(0)}^2\right] +  \frac{\eta(2\alpha n^{-\frac{3}{4}} +\eta)\sqrt{n}}{\alpha^2} \log \left( \frac{2n(2\alpha n^{-\frac{3}{4}}+\eta)}{\eta \lambda_0 B b_0} \right) \nonumber \\
    &= \mathbb{E}\left[\norm{\vy-\vu(0)}^2\right] +  \left(\frac{\eta^2\sqrt{n}}{\alpha^2}+\frac{2\eta n^{-\frac{3}{4}}}{\alpha}\right) \log \left( \frac{2n(2\alpha n^{-\frac{3}{4}}+\eta)}{ \lambda_0 B b_0} \right) \nonumber
\end{align}     
% \subsection{Proof of Lemma \ref{lem:adagrad_stochastic3}}
% Now back to inequality \eqref{eq:keycontraction1}, we have with high probability that $1-\delta'-\delta$ for $k> T_0$
% \begin{align}
% &\mathbb{E}\left[\norm{\vect{y}-\vect{u}(k+1)}^2 \right]  
%  \le \left(1-\frac{ \eta \lambda_0 \delta'}{2n\mathcal{Q}_{T_0} }  \right) \mathbb{E}\left[ \|\vy-\vu(k)\|^2   \right] 
% \end{align}
% Thus we have exponential convergence rate for all $t>T_0$. Note that the above inequality \eqref{eq:case1-b0-contraction-stoc} is analogue to \eqref{eq:case1-b0-contraction}. Thus we have $\mathbb{E} \left[ \norm{\vect{y}-\vect{u}(k+1)}^2 \right] \leq \varepsilon$ with high probability $1-\delta -\delta'$ after:
% \begin{align}
%     T &= \frac{2n}{\eta \lambda_0 \delta'} \left( b_{T_0} + \frac{2\alpha n^{-\frac{3}{4}} \sqrt{n}}{\eta {\lambda_0}B}\mathbb{E}\left[ \norm{\vy-\vu(T_0)}^2\right] + \sqrt{  \frac{\alpha^2 \mathbb{E}\left[ \|\vy-\vu(T_0)\|^2\right]}{\sqrt{ n}}}\right) 
% \end{align}




% \subsection{Proof for the Lemmas \ref{lem:adagrad_stochastic1}}

% \subsection{Solve for $T_0$}
% In this section, we will mainly discuss about $T_0$ when 







==> adagradstochastic.tex <==
% In this section, we analyze stochastic algorithms for optimizing neural networks. We begin with the vanilla SGD, $\vW{(k+1)} = \vW{(k)} - \eta \frac{\partial L_{\xi_k}(\vW{(k)})}{\partial \vW }$. At $kth$ iteration, the sample loss is
% %  \begin{align*}
% %    \frac{\partial L_{
% %    \xi_k}(\vW(k))}{\partial \vw_r} = \frac{1}{\sqrt{m}}
% %     (u_{\xi_k}(k)-y_{\xi_k})\vx_{\xi_k}\mathbb{I}_{\{\vw_r^T\vx__{
% %    \xi_k}\geq0\}}
% % \end{align*} 


%   $$ L_{\xi_{k}}(\vW(k))  = 
%      \frac{1}{2}( u_{\xi_k}(k)-y_{\xi_k})^2$$

% where $u_{\xi_k}(k) = \frac{1}{\sqrt{m}}\sum_{r=1}^{m}a_r
%      \sigma(\langle{\vw_r(k), \vx_{\xi_k} \rangle})$ and $ \xi_k \sim U(\left\{1,2,\ldots,n\right\})$. We have the following theorem for SGD with constant stepsize.
% \begin{thm} \label{thm:main_sgd} \textbf{(Convergence Rate of Stochastic Gradient Descent with Constant Stepsize)} Under the same setting as \cite{du2018gradient}, and standard  assumptions of the SGD algorithms (See Assumptions  \ref{asmp1},  \ref{asmp2}  and  \ref{asmp3}). 
% % \simon{What is the $m$ dependency?}
% Each sample $(x_{\xi_k},y_{\xi_k})$ is uniformly chosen with probability $\frac{1}{n}$. With over-parametrization $
% m = \Omega \left(\frac{n^8}{\lambda_0^4\delta^3\widetilde{\delta}}  \right)$ with high probability $1-\widetilde{\delta}$ , 
% % 	Set the stepsize 
% % $ \eta = \Theta \left ( \frac{1}{ \norm{\vH^{\infty}}} \right),$
% %  then with probability at least $1-\delta$
% %  over the random initialization, after
% % $T =\widetilde{O} \left({ \norm{ \vH^{\infty}}} \log\left( { 1 }/{ \varepsilon} \right)/{   \lambda_0 } \right) \text{ iterations, we have }
% % L(\mat{W}(T)) \le \varepsilon + \sum_{k=0}^{T}\left( 1-\frac{\lambda_0}{\|\vH^{\infty}\|}\right)^{k} \sigma_{T-k}+c. 
% % $
% if we set the stepsize to be 
% $ \eta = O \left ( \frac{\lambda_0}{n} \right),$
%  then with probability at least $1-\delta-\delta'$, after
% $
% T =\widetilde{O} \left( \frac{n^2}{   \lambda_0^2\delta' } \log\left( \frac{ 1 }{ \varepsilon} \right) \right)\text{ iterations, we have }
%  L(\mat{W}(T)) \le \varepsilon. 
% $
% \end{thm}
% The theorem implies that a major obstacle using vanilla SGD  for the loss converging to zero is the variance of the gradient. The large learning rate can only make the training error small but not to zero (see  Appendix \ref{sec:proof_sgd} for details). In order to have zero training error, one needs to set the learning rate to be much smaller, for example, $ \eta = O \left ( \frac{\lambda_0}{n} \right)$. Thus, in practice, learning rates with decaying schedules \citep{goyal2017accurate} or adaptive gradient methods are often used.

% , defined as 
% $\sum_{i=1}^n\mathbb{E}_{\xi_k}\left[\left( (u_{\xi_k}-y_{\xi_k})\mat{H}_{i\xi_ k}(k) -\frac{1}{n}\sum_{j=1}^n(u_j-y_j)\mat{H}_{ij}(k) \right)^2\right]$.\footnote{ $\mathbb{E}_{\xi_k}[\cdot ]$ means expectation over the random variable $\xi_k$ conditional on the random sequence $\{\xi_\ell\}_{\ell=1} ^{k-1}$, and $\mathbb{E}_{\xi_1,\cdots,\xi_k}[\cdot]$ over the  random sequence $\{\xi_\ell\}_{\ell=0}^k$.} 



\subsection{Stochastic AdaLoss for Two-layer Neural Network}
Even though over-parameterized neural networks share most of the properties of linear regression in deterministic setting, the connection is less strong in stochasic setting. In the remaining section, we state the convergence results for the two-layer neural networks using  stochastic \textbf{AdaLoss}:
\begin{align}
  \textbf{AdaLoss}\quad b_{k+1}^2 \leftarrow b_k^2 + \alpha^2\sqrt{n}( y_{\xi_k}-u_{\xi_k})^2.\label{alg:adagradloss-stochastic}
 \end{align}

% 	m = \Omega \left(\frac{n^8}{\lambda_0^4\delta^3} +  \frac{\eta^2 \|\vH^\infty\|^4 }{\alpha^2 \sqrt{n}} \left( \frac{ (\eta C\|\vH^\infty\|)^2-b_0^2}{\mu \gamma\varepsilon}+\frac{\delta}{\gamma}\right)\right).
% 	$
We first utilize the following assumption when $b_0$ is small.
\begin{asmp} \label{ruil2}
\textbf{$(\varepsilon, \mu_{\scaleto{NN}{4pt}}, \gamma)-$ Restricted Uniform Inequality of Loss for Neural Network (RUIL-NN):} $ \forall \varepsilon > 0$, $\exists (\mu_{\scaleto{NN}{4pt}}, \gamma)$ s.t. $\forall \vu \in \mathcal{D}_{\varepsilon} \triangleq \{ \vu \in \mathbb{R}^n: \| \vu-\vy\|^2 > \varepsilon\}$, $\mathds{P} ((u_{\xi_k}(k) - y_{\xi_k})^2 \geq \mu_{\scaleto{NN}{4pt}} \frac{\|\vu(k) - \vy\|^2}{n} ) \geq \gamma$, $\forall \xi_k \in [n]$.
\end{asmp}

Note that in neural network, RUIL-NN measures the uniform lower bound of the sample loss with respect to the average loss, in a restricted region $\mathcal{D}_{\varepsilon}$ . Compared with RUIL-LR, since $\|\vw-\vw^*\|^2 \geq 2/\bar{\lambda_1} \|\vX \vw - \vy\|^2$, where $\| \vX \vw-\vy\|$ is the total loss in linear regression, $\mu_{\scaleto{NN}{4pt}} = \mathcal{O}(\mu_{\scaleto{LR}{4pt}}/ \bar{\lambda_1})$.
	
\begin{thm}\textbf{(Stochastic AdaLoss: Convergence for Two-layer Network)}
	\label{thm:main_adagradloss_sto}
Under Assumption~\ref{asmp:norm1}, Assumption~\ref{asmp:lambda_0}, and Assumption \ref{ruil2}, $(\varepsilon, \mu_{\scaleto{NN}{4pt}}, \gamma)-$ RUIL-NN. If the width satisfies $
	m = \widetilde{\Omega} \left( \frac{n^8}{\lambda_0^4\delta^3\widetilde{\delta}} +\frac{\eta^2 n^5}{ \lambda_0^2\delta^2\alpha^4\widetilde{\delta}} \left(\frac{1}{\mu_{\scaleto{NN}{2pt}}\gamma \varepsilon} \left(\left(\frac{2n(2\alpha n^{-3/4} +\eta)}{\lambda_0 B}\right)^2 -b_0^2\right)+\frac{\delta_{NN}}{\gamma}\right)\right) 
	$ \footnote{$B = \Theta(1)$ (see Table 1 for expression)} with high probability $1-\widetilde{\delta} - \exp(-\frac{\|\Delta\|^2}{2(N\gamma(1-\gamma)+\delta_{NN})})$.
	Then Algorithm~\eqref{alg:adagradloss-stochastic}   admits  the following results.\\
		\textbf{(a)} If the hyper-parameter satisfies $ b_0 \geq \frac{2n(2\alpha n^{-3/4}+\eta)}{ \lambda_0 B}$, then with probability $1 - \delta'-\delta''$,
		$\min_{t\in [T]}\norm{\vect y- \vect u(t)}^2 \le\varepsilon$ 
			%$\norm{\vect y- \vect u(t)}^2 \le\varepsilon$ 
		after
		\begin{footnotesize}
				\begin{align*}
		T = \widetilde{O}\left(\frac{2n}{\eta \lambda_0 \delta'\delta''} \left( b_{0} + \frac{2\alpha^2 \sqrt{n}}{\eta {\lambda_0}B}\mathbb{E}\left[ \norm{\vy-\vu(0)}^2\right] + \sqrt{  \frac{\alpha^2 \mathbb{E}\left[ \|\vy-\vu(0)\|^2\right]}{\sqrt{ n}}} \right) \log\left(\frac{1}{\varepsilon} \right)\right).
		\end{align*}
		\end{footnotesize}
\textbf{(b)} If the hyper-parameter satisfies $ 0< b_0\leq \frac{2n(2\alpha n^{-3/4}+\eta)}{\lambda_0 B}$, then with probability $1-\delta -\delta'-\delta''- \exp(-\frac{\|\Delta\|^2}{2(N\gamma(1-\gamma)+\delta_{NN})})$,  $\min_{t\in [T]}\norm{\vect y- \vect u(t)}^2 \le\varepsilon$   after	
\begin{footnotesize}
     	\begin{align*}
		T = \widetilde{O}\left(\frac{\left(\frac{2n(2\alpha n^{-3/4} +\eta)}{\lambda_0 B}\right)^2 -b_0^2}{\varepsilon \mu_{\scaleto{NN}{2pt}}\gamma \delta''\alpha^2 \sqrt{n}} +\frac{\delta_{NN}}{\gamma \delta''\alpha^2 \sqrt{n}}
		+  \left(\frac{\alpha^2 n^{5/2}}{\eta^2 \lambda_0^2 \delta \delta'\delta''}+\frac{n^2+n^{\frac{3}{4}}\alpha/\eta}{\lambda_0^2 \delta'\delta''}\right) \log\left(\frac{1}{\varepsilon} \right)\right).
		\end{align*}   
\end{footnotesize}
\end{thm}
We would like to point out that the major challenge in the analysis is to deal with the correlation between the random variable $b_k$ and loss function $\|\vy-\vu(k)\|$ (see Appendix \ref{sec:adagrad_stoch}). We use the Markov Inequality to achieve the worse upper bound: the parameter $\delta$ is for random initialization, $\delta'$ is for $b_t$, $\delta''$ is for $\|\vy-\vu(k)\|$ and $\widetilde{\delta} $ is for $\|\vw_r-\vw_r(k)\|$.  Note that if $b_0 > \frac{2n(2\alpha n^{-3/4}+\eta)}{\lambda_0 B}$, then the order of AdaLoss in the stochastic setting is still the same as SGD with fixed stepsize. However, if $b_0 <\frac{2n(2\alpha n^{-3/4}+\eta)}{\lambda_0 B}$, the level of over-parametrization ($m$) heavily depends on the parameters in  Assumption \ref{ruil2}.  This assumption is crucial, as it is not clear how quickly  $b_t$ grows to the critical threshold $ \eta \bar{\lambda_1}$. By using probability in high dimensions (c.f. Assumption 4.2), we derive a worse iteration complexity for small initialization of $b_0$. The iteration complexity of stochastic AdaLoss for two-layer neural network is unfortunately  worse than that for linear regression. The key reason is that the two-layer neural network is highly non-convex, and one cannot utilize the property of convexity to obtain fast convergence. Note that the bound in our theorem is the worst bound without any assumption for the data distribution. We believe, practically, the bound could be much tighter.  

==> command.tex <==
%for convinience
\newcommand{\vct}{\boldsymbol}
\newcommand{\mat}{\mathbf}
\newcommand{\vect}{\mathbf}
\newcommand{\rnd}{\mathsf}
\newcommand{\ud}{\mathrm d}
\newcommand{\nml}{\mathcal{N}}
\newcommand{\loss}{\mathcal{L}}
\newcommand{\hinge}{\mathcal{R}}
\newcommand{\kl}{\mathrm{KL}}
\newcommand{\cov}{\mathrm{cov}}
\newcommand{\dir}{\mathrm{Dir}}
\newcommand{\mult}{\mathrm{Mult}}
\newcommand{\err}{\mathrm{err}}
\newcommand{\sgn}{\mathrm{sgn}}
%\renewcommand{\span}{\mathrm{span}}
%\newcommand{\argmin}{\mathrm{argmin}}
%\newcommand{\argmax}{\mathrm{argmax}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\conv}{\mathrm{conv}}
%\newcommand{\E}{\mathbb{E}}
\newcommand{\diag}{\mat{diag}}
\newcommand{\acc}{\mathrm{acc}}

\newcommand{\aff}{\mathrm{aff}}
\newcommand{\range}{\mathrm{Range}}
\newcommand{\Sgn}{\mathrm{sign}}

\newcommand{\hit}{\mathrm{hit}}
\newcommand{\cross}{\mathrm{cross}}
\newcommand{\Left}{\mathrm{left}}
\newcommand{\Right}{\mathrm{right}}
\newcommand{\Mid}{\mathrm{mid}}
\newcommand{\bern}{\mathrm{Bernoulli}}
\newcommand{\ols}{\mathrm{ols}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\opt}{\mathrm{opt}}
\newcommand{\ridge}{\mathrm{ridge}}
\newcommand{\unif}{\mathrm{unif}}
\newcommand{\Image}{\mathrm{im}}
\newcommand{\Kernel}{\mathrm{ker}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\pred}{\mathrm{pred}}
\newcommand{\distequal}{\stackrel{\mathbf{P}}{=}}
%\newcommand{\gege}{\textcircled{1}}
\newcommand{\gege}{{A(\vect{w},\vect{w}_*)}}
\newcommand{\gele}{{A(\vect{w},-\vect{w}_*)}}
\newcommand{\lele}{{A(-\vect{w},-\vect{w}_*)}}
\newcommand{\lege}{{A(-\vect{w},\vect{w}_*)}}
\newcommand{\firstlayer}{\mathbf{W}}
\newcommand{\firstlayerWN}{v}
\newcommand{\secondlayer}{a}
\newcommand{\inputvar}{\vect{x}}
\newcommand{\anglemat}{\mathbf{\Phi}}
\newcommand{\holder}{H\"{o}lder }
\newcommand{\preddiff}{\triangle}

\def\R{\mathbb{R}}
\def\Z{\mathbb{Z}}
\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cP{\mathcal{P}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
 \def\cW{\mathcal{W}}
\def\cZ{\mathcal{Z}}
\def\bP{\mathbf{P}}
\def\TV{\mathrm{TV}}
\def\MSE{\mathrm{MSE}}


\def\vb{\mathbf{b}}
\def\vw{\mathbf{w}}
\def\va{\mathbf{a}}
\def\vv{\mathbf{v}}
\def\vZ{\mathbf{Z}}
\def\vS{\mathbf{S}}

\def\dx{\textnormal{dx}}
\def\dy{\textnormal{dy}}
\def\dz{\textnormal{dz}}
\def\dt{\textnormal{dt}}
\def\d{\textnormal{d}}
\usepackage{hyperref}

% \usepackage{tcolorbox}

%\usepackage[font=small,labelfont=bf]{caption}

\usepackage{array}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\def\p#1#2{\frac{\partial #1}{\partial #2}}
\def\dotprod#1#2{\langle #1, #2\rangle}
\def\vx{\mathbf{x}}
\def\vy{\mathbf{y}}
\def\vw{\mathbf{w}}
\def\vW{\mathbf{W}}
\def\vI{\mathbf{I}}
\def\vwopt{\mathbf{w}_*}
\def\v0{\mathbf{0}}
\def\va{\mathbf{a}}
\def\vu{\mathbf{u}}
\def\vf{\mathbf{f}}
\def\ve{\mathbf{e}}
\def\vr{\mathbf{r}}
\def\vv{\mathbf{v}}
\def\vX{\mathbf{X}}
\def\vH{\mathbf{H}}
\def\vU{\mathbf{U}}
\def\vQ{\mathbf{Q}}
\def\vV{\mathbf{V}}
\def\vSi{\mathbf{\Sigma}}
\def\vbSi{\bar{\mathbf{\Sigma}}}
\def\vbU{\bar{\mathbf{U}}}
\def\vbV{\bar{\mathbf{V}}}
\def\vc{\mathbf{c}}
\def\vu{\mathbf{u}}
\def\vone{\mathbf{1}}
\def\vE{\mathbf{E}}
\def\proj{\mathrm{proj}}
\def\norm#1{\|#1\|}
\def\d{\mathrm{d}}
\def\d#1{\mathrm{d}#1}
\def\d#1#2{\frac{\  mathrm{d}#1}{\mathrm{d}#2}}
% \def\g#1{\partial#1}
\def\g#1{g_{#1}}

\def\dd{\mathrm{d}}

\def\jbn#1{{J^{BN}(#1)}}
\def\s#1{S(#1)}

\def\hvx{\hat \vx}
\def\tvx{\tilde \vx}
\def\tvone{\tilde \vone}

\def\X#1{X^{(#1)}}
\def\w#1{\mathbf{w}^{(#1)}}

% \def\vphi{\mathbf{\phi}}
\def\vphi{\boldsymbol{\phi}}  
\def\veps{\boldsymbol{\epsilon}}

\def\tvphi{\tilde{\vphi}}
\def\dtvphi{\dot{\tilde{\vphi}}}
\def\dhvphi{\dot{\hat{\vphi}}}
\def\tvr{\tilde\vr}

\def\etal{{\textit{et~al.~}}}

%\newcommand{\mat}[1]{\mathbf{#1}}
%\newcommand{\vect}[1]{\mathbf{#1}}  \newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\expect}{\mathbb{E}}
\newcommand{\prob}{\mathbb{P}}
\newcommand{\prox}[2]{\textbf{Prox}_{#1}\left\{#2\right\}}
\newcommand{\event}[1]{\mathscr{#1}}
%\newcommand{\set}[1]{#1}
\newcommand{\diff}{\text{d}}
\newcommand{\difference}{\triangle}
\newcommand{\inputdist}{\mathcal{Z}}
\newcommand{\indict}{\mathbb{I}}
\newcommand{\rotmat}{\mathbf{R}}
\newcommand{\normalize}[1]{\overline{#1}}
\newcommand{\vectorize}[1]{\text{vec}\left(#1\right)}
\newcommand{\vclass}{\mathcal{G}}
\newcommand{\pclass}{\Pi}
\newcommand{\qclass}{\mathcal{Q}}
\newcommand{\rclass}{\mathca  l{R}}
\newcommand{\classComplexity}[2]{N_{class}(#1,#2)}
\newcommand{\cclass}{\mathcal{F}}
\newcommand{\gclass}{\mathcal{G}}
\newcommand{\pthres}{p_{thres}}
\newcommand{\ethres}{\epsilon_{thres}}
\newcommand{\eclass}{\epsilon_{class}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\lowprobstate}{\psi}
\newcommand{\actions}{\mathcal{A}}
\newcommand{\contexts}{\mathcal{X}}
\newcommand{\edges}{\mathcal{E}}
\newcommand{\variance}{\text{Var}}
\newcommand{\params}{\vect{w}}

\newcommand{\relu}[1]{\sigma\left(#1\right)}
\newcommand{\reluder}[1]{\sigma'\left(#1\right)}
\newcommand{\act}[1]{\sigma\left(#1\right)}




==> discussion.tex <==
In this section, we compare our proposed algorithm AdaLoss with existing adaptive methods.
Algorithm  \ref{alg:adagradloss} can be viewed as a variant of the standard AdaGrad algorithm proposed by  \cite{duchi2011adaptive}, where the norm version of the update is
\begin{align*}
 b_{k+1}^2 = b_{k}^2 + \sqrt{m} \max_{r\in[m]} \bigg\| \frac{\partial L(\vW{(k)})}{\partial \vw_r } \bigg\|^2. 
\end{align*}
Our algorithm AdaLoss is similar to AdaGrad, but is distinctly different from AdaGrad: we update $b_{k+1}^2$ using the \emph{norm} of the \emph{loss} instead of the \emph{squared norm} of the \emph{gradient}.  We considered the AdaLoss update instead of AdaGrad because, in the setting considered here, the modifications allowed for dramatically better theoretical convergence rate. 

\paragraph{Why the Loss instead of the Gradient?}  Indeed, our update of $b^2_{k+1}$ is not too different from the following update rule using the gradient 
\begin{align}
b_{k+1}^2 = b_{k}^2 + \alpha^2\sqrt{m} \max_{r\in[m]} \bigg\| \frac{\partial L(\vW{(k)})}{\partial \vw_r } \bigg\|.
\label{eq:adagradss}
\end{align}
The AdaLoss update can be upper and lower  bounded   by $b_k^2$ and the norm of the gradient, i.e.,
\[   b_{k}^2 +  \alpha^2 \sqrt{m} \max_{r\in[m]}\bigg\| \frac{\partial L(\vW{(k)})}{\partial \vw_r } \bigg\|\leq b_{k+1}^2 \leq b_{k}^2 + \frac{ \alpha^2 \sqrt{m}}{\sqrt{\lambda_0}} \max_{r\in[m]}\bigg\| \frac{\partial L(\vW{(k)})}{\partial \vw_r } \bigg\| \]
where the first and second inequalities are respectively due to Proposition \ref{prop:a1} and  Proposition \ref{lem:grad_to_training_sub}. 
%\simon{Write a formal lemma and refers to it. Using \textbf{P1} looks weird to me}.
\begin{prop}
\label{lem:grad_to_training_sub}
If $\lambda_{min} (\vH)\geq \frac{\lambda_0}{2}$, then $\|\vy -\vu\| \leq \frac{ \sqrt{2m}}{\sqrt{\lambda_0}}\max_{r\in[m]}\| \frac{\partial L (\vW)}{\partial \vw_r}\|.$ \footnote{Proof  is given in Appendix \ref{sec:proof_prop} } 
\end{prop}
However, we use $\sqrt{n}\|\vy-\vu(k) \|$ instead of using the gradient to update $b_k$ because our convergence  analysis requires  lower and upper bounding the dynamics $b_1, \ldots, b_{k}$, in terms of $\|\vy-\vu(k) \|$. If $b_k$ were instead updated using  \eqref{eq:adagradss}, then 
%$b_{k+1}^2$ lower bounded by
$$b_{k+1}^2\geq b_{k}^2 + \frac{ \alpha^2}{\sqrt{2\lambda_0}} \max_{r\in[m]} \bigg\| \frac{\partial L(\vW{(k)})}{\partial \vw_r } \bigg\|.$$
The above lower bound of $b_k$ results in a larger $T$ in Case (2) by a factor of $\sqrt{n/\lambda_0}$.  Using the loss instead of the gradient to update $b_k$ is independently useful as reusing the already computed loss information for each iteration can save some computation cost and thus make the update more efficient.

\paragraph{Why the norm and not the squared-norm?}  For ease of comparison with Algorithm \ref{alg:adagradloss}, we switch from gradient information to loss and compare with two close variants: 
\begin{align}
b_{k+1}^2 = b_{k}^2 +  \alpha^2 \sqrt{n}\|\vy-\vu(k) \| ^2 \label{eq:adagradss1} \\
b_{k+1} = b_{k} + \alpha \sqrt{n}\|\vy-\vu(k) \| 
\label{eq:adagradss2}.
\end{align}
Equation \eqref{eq:adagradss1} using the ``square'' rule update  is the standard AdaGrad proposed by  \cite{duchi2011adaptive} and has been widely recognized as important optimizer in deep learning -- especially for training sparse datasets. For our over-parameterized models, this update rule does give a better convergence result in Case 1 when $b_0/\eta \geq  C \|\vH^{\infty}\|$ \footnote{The convergence proof is straightforward and similar to the first case in Theorem \ref{thm:main_adagradloss}}. However,  when the initialization  $b_0/\eta\leq  C \|\vH^{\infty}\|$, we were only able to prove convergence in case the level of  over-parameterization (i.e., $m$) depends on the training error $1/\varepsilon$, the bottleneck resulting from the attempting to prove the analog of Lemma \ref{lem: small_w_for_allbsq1_sub} (see Proposition \ref{prop:adasq} below).

 \begin{prop}\label{prop:adasq}
Let  $T_0\geq 1$ be the first index such that $b_{T_0} \geq  \eta C \|\vH^{\infty}\| $. Consider the update of $b_{k}$ in \eqref{eq:adagradss1}.
Then for every $r \in [m]$, we have  for $k=0,1,\ldots,T_0-1$,
\begin{align*}
\|\vw_r(k+1)-\vw_r(0)\|_2
&\leq   \frac{\eta\sqrt{2(k+1)}}{\alpha^2 \sqrt{m}}\sqrt{  1+ 2\log \left(\frac{C \eta \|\vH^{\infty}\| }{b_0}\right)}.
\end{align*}
\end{prop}
On the other hand, the update rule in \eqref{eq:adagradss2} can resolve the problem because the growth of $b_k$ is larger than \eqref{eq:adagradss1} such that the upper bound of $\|\vw_r(k)-\vw_r(0)\|_2$ $k=0,1\ldots,T_0-1$, is better than that in Proposition \ref{prop:adasq} and even Lemma \ref{lem: small_w_for_allbsq1_sub} if $c<b_0<  \eta C \|\vH^{\infty}\|$ for some small $c$. However, the growth of $b_k$ remains too fast once the critical value of $\eta C \|\vH^{\infty}\|$ has been reached -- the upper bound $b_{\infty}$ we were able to show is exponential in $1/\lambda_0$ and also in the hyper-parameters $b_0$,$\eta$, $\alpha$ and $n$, resulting in an extremely large  $T$ compared to Case (2) in Theorem \ref{thm:main_adagradloss}.



==> linear_proof.tex <==

We can rewrite the linear regression problem  \eqref{eq:linear} as
\begin{align}
args\min_{\vw \in \mathbb{R}^{d} } \frac{1}{2n}\|U\Sigma^{\frac{1}{2}} V(\vw-\vw^*)\|^2 =args \min_{V\vu\in \mathbb{R}^{d} } \frac{1}{2n}\|\Sigma^{\frac{1}{2}} (\hat{\vw}-\hat{\vw}^*)\|^2,  \label{eq:svd}
\end{align}
where $\hat{\vw} = V^\top\vw $. Let $[\hat{\vw}_{t+1}]_i$ denotes the entry of the $i$-th dimension of the vector. The standard gradient descent methods using the  adaptive stepsize $\eta_t$ is 
\begin{align}
[\hat{\vw}_{t+1}]_i =&  [\hat{\vw}_{t}]_i - \frac{\eta_t \lambda_i}{nb_t}([\hat{\vw}_{t}]_i -[\hat{\vw}^{*}]_i  ) \quad \text{with } b_{t+1}^2 =b_{t}^2 + \frac{1}{n^2} {\sum_{i=1}^n\lambda_i([\hat{\vw}_{t}]_i -[\hat{\vw}^{*}]_i  )^2} \label{eq:update_u}
\end{align}
%which implies that
%\begin{align*}
%\left([\hat{\vw}_{t+1}]_i-[\hat{\vw}^{*}]_i\right)^2  =&\left( 1 - \frac{\eta_t  \lambda_i}{nb_t} \right)^2([\hat{\vw}_{t}]_i -[\hat{\vw}^{*}]_i  )^2 .
%\end{align*}
%
%Let $s_{t}^{(i)} = \left([\hat{\vw}_{t}]_i-[\hat{\vw}^{*}]_i\right)^2 $. 
%As long as $\eta_t \leq \frac{2n}{\lambda_1}, \forall t$, then $\{\|\hat{\vw}_{t+1}-\hat{\vw}^{*}\|^2\}_{t\geq0}$  is a decreasing sequence. 
Note that \eqref{eq:update_u} can be equivalently written as
\begin{align}
s_{t+1}^{(i)} :=\left([\hat{\vw}_{t+1}]_i-[\hat{\vw}^{*}]_i\right)^2  =&\left( 1 - \frac{\eta \lambda_i}{nb_{t+1}} \right)^2([\hat{\vw}_{t}]_i -[\hat{\vw}^{*}]_i  )^2 \label{eq:exact-dynamic}.
\end{align}
We will  be using the following key  inequalities:
\begin{align}
\| \vw_{t+1}-\vw^*\|^2
&\leq \left( 1-\frac{2\eta \lambda_n}{nb_{t+1}} \left(1- \frac{\eta \lambda_1}{2nb_{t+1}}\right) \right)\| \vw_{t}-\vw^*\|^2\label{eq:ineq2}\\
\| \vw_{t+1}-\vw^*\|^2
&\leq  \left( 1- \frac{2\eta \lambda_1 \lambda_n}{ (\lambda_n+\lambda_1)nb_{t+1}}\right)\|\vw_{t}-\vw^*\|^2 \nonumber\\
&\quad  +\frac{\eta}{nb_{t+1}} \left(\frac{\eta}{nb_{t+1}}- \frac{2}{\lambda_n +\lambda_1}\right)\| X^\top X\left(\vw_{t}-\vw^*\right)\|^2   \label{eq:ineq3}\\
\| X\left( \vw_{t+1}-\vw^*\right)\|^2
%&= \| X \left( \vw_{t}-\vw^*\right) -\frac{\eta}{b_{t+1}} X X^\top X \left( \vw_{t}-\vw^*\right) \|^2  \nonumber\\ 
&\leq \left(1- \frac{2\eta}{nb_{t+1}} \left( 1 - \frac{\eta\lambda_1}{2nb_{t+1}} \right) \right)\| X^\top X \left(\vw_{t}-\vw^*\right)\|^2   \label{eq:ineq1}
\end{align}
Based on the above fact, we first present the easy convergence case  when $n b_0\geq\eta\lambda_1/2$ and then we will analyze the case when $n b_0\leq\eta\lambda_1/2$.

\begin{lem}
\label{lem:increase_sub}\textbf{ (Linear Convergence Rate  if $b_0 \geq \frac{\eta\lambda_1}{ 2n}$)}
Consider  the problem \eqref{eq:linear}  and the adaptive gradient descent  method \eqref{eq:adalinear}.  Suppose there exists the unique $\vw^*$ such that $\vy=X\vw^*$ and suppose $X^TX$ is a positive definite matrix  with singular value decomposition $X^TX = U\Sigma V$  where  the diagonal values of $\Sigma$ have the arrangement $  \lambda_1\geq \lambda_2\geq\ldots\geq  \lambda_n>0$. Assume $\| \vw_{0}-\vw^*\|^2\neq0$. If $n b_0 \geq \eta\lambda_1/2$,   we have $\| \vw_{T}-\vw^*\|^2\leq \epsilon$ for
\begin{align}
T= \max \left\{ \widetilde{T},  \frac{\lambda_1}{\lambda_n}\left( 1+  \frac{\| X \left(\vw_{0}-\vw^*\right)\|^2}{\lambda_1 \eta^2} \right)\right\}\log\left( \frac{\| \vw_{0}-\vw^*\|^2}{\epsilon}\right)
\end{align}
%
\begin{align*}
\text{where } \quad \widetilde{T} &:= \max \left\{ \frac{ (nb_1)^2}{\lambda_n\left(2nb_1-\eta \lambda_1\right)} \mathbbm{1}_{ \left\{ b_1\in\left(\frac{ \eta \lambda_1}{2n}, \frac{ \eta( \lambda_1+\lambda_n) }{2n}\right) \right\} },   \frac{ (\lambda_1+\lambda_n )^2}{ 4 \lambda_1\lambda_n } \right\}\\
 \text{with }  &\quad b_1 = \sqrt{b_0^2 + \frac{1}{n^2}\|X^TX(\vw_0-\vw^*)\|^2} > b_0\geq \frac{\eta \lambda_1}{2} 
\end{align*}
%
%\text{or } & T = \label{eq:second-phase}
%\end{align}

\end{lem}
\begin{proof}
We have that $b_t$ eventually stabilizes  in following 3 regions: 
 (a) $ \frac{\eta\lambda_1}{2}\leq  n b_t< \frac{ \eta \left(\lambda_1+\lambda_n\right)}{2},$
(b) $ nb_t\geq \frac{ \eta \left(\lambda_1+\lambda_n\right)}{2},$
and   (c) $ nb_t\geq \eta \lambda_1.$ Based on the above fact, we will prove  two exponential convergence rate.
%Start with the equality  of \eqref{eq:exact-dynamic}:
%\begin{align}
%\left([\hat{\vw}_{t+1}]_i-[\hat{\vw}^{*}]_i\right)^2 =&\left( 1 - \frac{\eta \lambda_i}{nb_{t+1}} \right)^2\left([\hat{\vw}_{t}]_i-[\hat{\vw}^{*}]_i\right)^2 \nonumber\\
%=&  \left([\hat{\vw}_{t}]_i-[\hat{\vw}^{*}]_i\right)^2 - \frac{2\eta \lambda_i}{nb_{t+1}} \left(1- \frac{\eta \lambda_i}{2nb_{t+1}}\right)  \left([\hat{\vw}_{t}]_i-[\hat{\vw}^{*}]_i\right)^2  \nonumber\\
%\leq& \left([\hat{\vw}_{t}]_i-[\hat{\vw}^{*}]_i\right)^2 - \frac{2\eta \lambda_n}{nb_{t+1}} \left(1- \frac{\eta \lambda_1}{2nb_{t+1}}\right) \left([\hat{\vw}_{t}]_i-[\hat{\vw}^{*}]_i\right)^2 \label{eq:contr}
%\end{align}
\\
For all $t$ such that $\frac{\eta\lambda_1}{2}\leq  n b_t\leq  \frac{ \eta \left(\lambda_1+\lambda_n\right)}{2}$, then from inequality \eqref{eq:ineq2}
\begin{align}
\| \vw_{t+1}-\vw^*\|^2
&\leq \left( 1-\frac{2\eta \lambda_n}{nb_{t+1}} \left(1- \frac{\eta \lambda_1}{2nb_{t+1}}\right) \right)\| \vw_{t}-\vw^*\|^2 \nonumber\\
&\leq  \left( 1-\frac{2 \eta \lambda_n}{nb_1} \left(1- \frac{\eta \lambda_1}{2nb_{1}}\right) \right)\| \vw_{t}-\vw^*\|^2 \nonumber\\
%&\leq \left(\frac{\eta \lambda_1}{nb_{1}} -1\right)^2\| \vw_{t}-\vw^*\|^2 \nonumber \\
&\leq \exp\left(-\frac{2\eta \lambda_n}{nb_1}  \left(1-\frac{\eta \lambda_1}{2nb_{1}}\right)\right)\| \vw_{t}-\vw^*\|^2\label{eq:first-bound}.
\end{align}
%\begin{align}
%\| \vw_{t+1}-\vw^*\|^2
%&\leq \left( 1-\frac{2\eta \lambda_n}{nb_{t+1}} \left(1- \frac{\eta \lambda_1}{2nb_{t+1}}\right) \right)\| \vw_{t}-\vw^*\|^2 \nonumber\\
%&\leq \left(\frac{\eta \lambda_1}{nb_{t+1}}-1\right)^2\| \vw_{t}-\vw^*\|^2 \nonumber\\
%&\leq \left(\frac{\eta \lambda_1}{nb_{0}} -1\right)^2\| \vw_{t}-\vw^*\|^2 \nonumber \\
%&\leq \exp\left(- 2\left(2-\frac{\eta \lambda_1}{nb_{0}}\right)\right)\| \vw_{t}-\vw^*\|^2\label{eq:first-bound}.
%\end{align}
It  implies  that after 
\begin{align*}
T_0 =  \frac{ n^2b_0^2 +\|X^TX(\vw_0-\vw^*)\|^2}{ \eta\lambda_n\left(2 \sqrt{ b_0^2+\|X^TX(\vw_0-\vw^*)\|^2}-\eta \lambda_1\right)}\log\left( \frac{\| \vw_{0}-\vw^*\|^2}{\epsilon}\right),\quad \text{if}\quad  n b_{T_1}\leq \frac{\eta (\lambda_1+\lambda_n)}{2},
\end{align*}
then $\| \vw_{T_0}-\vw^*\|^2\leq \epsilon$. However, after $T_0$, it is possible that $nb_{T_0}> \frac{\eta (\lambda_1+\lambda_n)}{2}$.  We then continue to analyze case (b) and then (c).\\
Suppose there exists index $M_1$ such that  $ \frac{ \eta \left(\lambda_1+\lambda_n\right)}{2}<n b_{t+1} \leq \eta\lambda_1$  for all $t\geq M_1$. The inequality  \eqref{eq:ineq3} reduces to
\begin{align*}
\| \vw_{t+1}-\vw^*\|^2
&\leq  \left( 1- \frac{2\eta \lambda_1 \lambda_n}{ nb_{t+1}(\lambda_n+\lambda_1)}\right)\|\vw_{t}-\vw^*\|^2 \nonumber\\
&\leq  \left( 1-\frac{2\lambda_n}{ (\lambda_n+\lambda_1)}\right) ^{t-M_1}\|\vw_{M_1}-\vw^*\|^2 \nonumber\\
&\leq  \left( 1-  \frac{2 \lambda_n}{ (\lambda_n+\lambda_1)}\right) ^{t-M_1}\left(1-\frac{2\lambda_n}{nb_1}  \left( 1-\frac{\eta \lambda_1}{2nb_{1}}\right)\right)^{M_1}\|\vw_{0}-\vw^*\|^2 \nonumber\\
 &\leq \left( 1 - \frac{1}{D_1}\right)^{t} \| \vw_{0}-\vw^*\|^2 
\end{align*}
where at the last step we  define the $D_1 $ as follows
%$\frac{1}{D} = \min \left\{\frac{2\lambda_n}{nb_0}  \left( 1-\frac{\eta \lambda_1}{2nb_{0}}\right), \frac{\eta \lambda_n}{nb_{\max} } \right\} < 1$ with $D$ bounded by
$$ D_1:=  \max \left\{ \frac{ (nb_1)^2}{\lambda_n\left(2nb_1-\eta \lambda_1\right)} \mathbbm{1}_{ \left\{ b_1\in\left(\frac{ \eta \lambda_1}{2n}, \frac{ \eta( \lambda_1+\lambda_n) }{n}\right) \right\} },   \frac{\lambda_1+\lambda_n}{ 2 \lambda_n } \right\}$$
%\begin{align}
%\text{either } & T =   \frac{nb_0}{2\left(2nb_0-\eta \lambda_1\right)}\log\left( \frac{\| \vw_{0}-\vw^*\|^2}{\epsilon}\right),\quad \text{if}   \label{eq:first-phase}
%\end{align}
%First bound \eqref{eq:first-phase} is obtained.
It  implies  that after 
\begin{align*}
T_1 = D_1\log\left( \frac{\| \vw_{0}-\vw^*\|^2}{\epsilon}\right),\quad \text{if } n b_{T_1} \in \left(\frac{ \eta \left(\lambda_1+\lambda_n\right)}{2n},\eta\lambda_1\right),
\end{align*}
then $\| \vw_{T_1+1}-\vw^*\|^2\leq \epsilon$. However, after $T_1$, it is possible that $nb_{T_1}> \eta \lambda_1$.  We then continue to analyze (c).\\

For case (c), suppose there exists index $M_2$,  the monotone increasing sequence $\{b_t\}_{t=0}^{\infty}$ satisfies  $nb_{M_2+1}\geq \eta \lambda_1$ and $nb_{M_2}<\eta \lambda_1$. Our strategy to obtain the exponential decay in $\| \vw_{t+1}-\vw^*\|^2$ for $t>M_2$ is to ensure that the limit of  $b_{t} $ is a finite number  as in \cite{ward2018adagrad} and \cite{wu2018wngrad}.
First,  we rewrite the update of  $b_t$ and have
%\begin{align} 
%b_{t+1} = b_{t} +\frac{1}{b_{t}+b_{t+1}} \frac{1}{n^2} \| X^\top X\left(\vw_t-\vw^* \right) \|^2 \nonumber
% \end{align}
\begin{align} 
b_{t+1} &= b_{t} +\frac{1}{b_{t}+b_{t+1}} \frac{1}{n^2} \| X^\top X\left(\vw_t-\vw^* \right) \|^2 \nonumber\\
&\leq  b_{t} +\frac{1}{n^2} \frac{\|X^\top X\left(\vw_\ell-\vw^*\right) \|^2}{b_{t+1}} \nonumber\\
&\leq  b_{M} +\frac{1}{n^2} \sum_{\ell=M}^t\frac{\|X^X(\vw_\ell-\vw^*) \|^2}{b_{\ell+1}}  \label{eq:bt}
\end{align}
We now need to bound above summation. For $nb_{t+1} \geq \eta\lambda_1, t\geq M_2$, inequality  \eqref{eq:ineq1} reduces to
\begin{align}
\| X\left( \vw_{t+1}-\vw^*\right)\|^2
&\leq \| X \left( \vw_{t}-\vw^*\right)\|^2- \frac{\eta}{nb_{t+1}}\| X^\top X \left(\vw_{t}-\vw^*\right)\|^2    \quad \text{ since } nb_{t+1}\geq \eta \lambda_1\nonumber\\ 
&\leq \| X \left( \vw_{M_2}-\vw^*\right)\|^2 - \sum_{\ell=M_2}^t\frac{\eta}{nb_{\ell+1}}\| X^\top X \left(\vw_{t}-\vw^*\right)\|^2 \nonumber
\end{align}
Rearranging above inequality and letting $t \rightarrow \infty$, we have
\begin{align}
\Rightarrow&\sum_{\ell=M_2}^\infty\frac{\| X^\top X \left(\vw_t-\vw^*\right) \|}{b_{\ell+1}}  \leq \frac{n}{\eta}\|X\left( \vw_{M_2}-\vw^*\right)\|^2 \leq  \frac{n}{\eta}\| X \left(\vw_{0}-\vw^*\right)\|^2 \label{eq:b}
\end{align} 
where at the last inequality we apply the  decreasing $\| X \left(\vw_{t}-\vw^*\right)\|^2$ for $b_t\geq \frac{\eta\lambda_1}{2n}$ based on \eqref{eq:ineq1} .

Returning to \eqref{eq:bt}, we can obtain the finite upper bound of $b_{t}$
\begin{align*}
\lim_{t \rightarrow \infty}b_{t}\leq  \frac{\eta\lambda_1}{n} \left(1 +  \frac{1}{\eta^2}\frac{\| X \left(\vw_{0}-\vw^*\right)\|^2}{\lambda_1}\right) \triangleq b_{\max} 
\end{align*}
Now, recall  the contraction formula \eqref{eq:ineq2} , we have $t>M_2$
\begin{align*}
\| \vw_{t+1}-\vw^*\|^2
&\leq\left( 1-\frac{2\eta \lambda_n}{nb_{t+1}} \left(1- \frac{\eta \lambda_1}{2nb_{t+1}}\right) \right)\| \vw_{t}-\vw^*\|^2 \nonumber\\ 
&\leq \left( 1 - \frac{\eta \lambda_n}{nb_{\max} }\right)\| \vw_{t}-\vw^*\|^2\quad \text{ since } nb_{\max} \geq nb_{t+1}\geq \eta \lambda_1\nonumber\\ 
 &\leq \left( 1 - \frac{\eta \lambda_n}{nb_{\max} }\right)^{t-M_2}\| \vw_{M_2}-\vw^*\|^2 \\
  &\leq \left( 1 - \frac{\eta \lambda_n}{nb_{\max} }\right)^{t-M_2}\left(1- \frac{1}{D_1}\right)^{M_2}\| \vw_{0}-\vw^*\|^2 \\
  &\leq \left( 1 - \frac{1}{D_2}\right)^{t} \| \vw_{0}-\vw^*\|^2 
\end{align*}
where at the last step we  define the $D_2 $ as follows
%$\frac{1}{D} = \min \left\{\frac{2\lambda_n}{nb_0}  \left( 1-\frac{\eta \lambda_1}{2nb_{0}}\right), \frac{\eta \lambda_n}{nb_{\max} } \right\} < 1$ with $D$ bounded by
$$ D_2 :=  \max \left\{D_1,  \frac{\lambda_1}{\lambda_n}\left( 1+  \frac{\| X \left(\vw_{0}-\vw^*\right)\|^2}{\lambda_1 \eta^2} \right)\right\}$$
Therefore, we have that $\| \vw_{T_2+1}-\vw^*\|^2\leq \epsilon$ after
\begin{align*}
T_2 = \frac{D_2}{2} \log\left( \frac{\| \vw_{0}-\vw^*\|^2}{\epsilon}\right)
\end{align*}
Note that the above bound $T_2 \geq T_1 \geq T_0$, thus we have the statement.
\end{proof}


 
\subsection{Exponential Increase of  $b_t$ from Small Initialization}
In this section, we first prove that it only takes very short steps for $b_t$ reach the critical value $\frac{\eta \lambda_1}{2n}$ if $b_0\leq \lambda_1/2n$. Then we explicitly characterize the increase of $\|\vw_t -\vw^*\|$ for $t\in \{\ell, b_\ell\leq \lambda_1/2n\}$ and conclude the linear convergence.
\begin{lem}
\label{lem:increase_sub}  \textbf{ (Exponential Increase for  $b_0 < \frac{\eta\lambda_1}{ 2n}$)}
Consider  the problem \eqref{eq:linear}  and the adaptive gradient descent  method \eqref{eq:adalinear}.  Suppose there exists the unique $\vw^*$ such that $\vy=X\vw^*$ and suppose $X^TX$ is a positive definite matrix  with singular value decomposition $X^TX = U\Sigma V$  where  the diagonal values of $\Sigma$ have the arrangement $  \lambda_1\geq \lambda_2\geq\ldots\geq  \lambda_n>0$.  Suppose we start with small initialization: $0<b_0< \lambda_1/2n$. Then there exists the first index $N$ such that $b_{N+1}\geq \lambda_1/2n$ and $b_N< \lambda_1/2n$, and  $N$  satisfies
\begin{align}
N \leq \bigg \lceil{ \log  \left(  1+
\frac{ \left({\eta \lambda_1} \right)^2 - 4(nb_0)^2 }{\eta^2 \lambda_1^2 }
\right) / \log \left (1+   \frac{ 4}{ \eta^2 \lambda_1 } \left([V^T\vw_{0}]_1 -[V^T\vw^{*}]_1 \right)^2 \right)\bigg \rceil} +1 \label{eq:TheN1}
\end{align}
There exists second index $M$ such that $b_{N+M+1}\geq \frac{\lambda_1+\lambda_n}{2n}$ and $b_{N+M}< \lambda_1/2n$, and $M$ satisfies
\begin{align}
M \leq \bigg \lceil{ \log  \left(  1+
\frac{ \left({\eta \lambda_1} \right)^2 - 4(nb_0)^2 }{\eta^2 \lambda_1^2 }
\right) / \log \left (1+   \frac{ 4}{ \eta^2 \lambda_1 } \left([V^T\vw_{0}]_1 -[V^T\vw^{*}]_1 \right)^2 \right)\bigg \rceil} +1 \label{eq:TheN2}
\end{align}

\end{lem}
\begin{proof}
% Denote the singular value decomposition $X^TX = U\Sigma V$  where each element of the diagonal $\Sigma$ have the arrangement $  \lambda_1\geq \lambda_2\geq\ldots\geq  \lambda_n$.  
%
%\[
%\Sigma =\begin{bmatrix}
%\lambda_1& 0 & \cdots & 0\\
%0 &\lambda_2 & \cdots & 0\\
%\vdots &\vdots & \vdots & \vdots\\
%0 &0 &  \cdots&\lambda_n\\
%\end{bmatrix}
%\quad 
%\text{with} \quad  \lambda_1\geq\lambda_2\geq\ldots\geq \lambda_n
%\]
%Suppose  $\lambda_n>0$ and there exists $\vw^*$ such that $\vy=X\vw^*$. Then 
Start with the fact in \eqref{eq:exact-dynamic}
\begin{align}
s_{t+1}^{(i)} :=\left([\hat{\vw}_{t+1}]_i-[\hat{\vw}^{*}]_i\right)^2  =&\left( 1 - \frac{\eta \lambda_i}{nb_{t+1}} \right)^2([\hat{\vw}_{t}]_i -[\hat{\vw}^{*}]_i  )^2. \label{eq:begin}
\end{align}
Observe that each $i$th sequence $\{s_{t}^{(i)}\}_{t=0}^k$ is monotone increasing  up to  $b_{k} \leq \frac{\eta \lambda_i}{2n}$.
%Suppose at $k$ iteration,  then the $i$-the sequence $\{s_{t}^{(i)}\}_{t=0}^k$ are monotone increasing sequence for all $i\in[n]$ since $\lambda_1\geq \lambda_2>\cdots\geq \lambda_n$.
%After $N$ iteration, suppose $b_N$ grows to the value such that $ \frac{\eta \lambda_2}{2} \leq b_{N} \leq \frac{\eta \lambda_1}{2}$ , then $\{s_{t}^{(i)}\}_{t=0}^{k}$   for all $i\in[n] / \{1\}$ are no longer monotone, while the sequence $\{s_{t}^{(1)}\}_{t=0}^N$ is still a monotone increasing sequence.  
In particular, if  $b_{0} \leq \frac{\eta \lambda_1}{2n}$ and after some $N$ such that $b_{N+1} \geq \frac{\eta \lambda_1}{2n}$ and $b_{N} \leq \frac{\eta \lambda_1}{2n}$, then we have the increasing sequence  of $\left([\hat{\vw}_{t}]_1-[\hat{\vw}^{*}]_1\right)^2, t =0, 1,\ldots,N$ not including  $\left([\hat{\vw}_{N+1}]_1-[\hat{\vw}^{*}]_1\right)^2$.  
We can estimate the number of step $N$ for $b_t$ grows to $b_{N+1}\geq\frac{\eta \lambda_1}{2n}$ from $b_0<\frac{\eta \lambda_1}{2n}$ and  $b_N< \frac{\eta \lambda_1}{2n}$   as follows
\begin{align}
\left( \frac{\eta \lambda_1}{2n} \right)^2 > b_{N}^2  & = b_{0}^2 + \sum_{t=0}^{N}  {\sum_{i=1}^n \frac{ \lambda_i}{n^2} ([\hat{\vw}_{t}]_i -[\hat{\vw}^{*}]_i  )^2}\notag\\
& \geq b_{0}^2 + \sum_{t=0}^{N}  \frac{ \lambda_1}{n^2} \left([\hat{\vw}_{t}]_1 -[\hat{\vw}^{*}]_1 \right)^2\notag\\  
&= b_{0}^2 +  \frac{ \lambda_1}{n^2}\left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2 \sum_{t=0}^{N}  \prod_{\ell=0}^t  \left( 1 - \frac{\eta \lambda_1}{ nb_{\ell}} \right)^{2}  \nonumber\\
&\geq b_{0}^2 +  \frac{ \lambda_1}{n^2} \left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2 \sum_{t=0}^{N-1}  \left( 1 - \frac{\eta \lambda_1}{ n b_{N-1}} \right)^{2t} 
 \label{eq:sum_term}
\end{align}
Since we have that
\begin{align}
&\left( \frac{\eta \lambda_1}{n} \right)^2  >  4b_N^2  \geq  4b_{N-1}^2+  \frac{ 4\lambda_1}{n^2} \left( [\hat{\vw}_{N-1}]_1 -[\hat{\vw}^{*}]_1 \right)^2 \nonumber\\
\Rightarrow \left( \frac{\eta \lambda_1}{ n b_{N-1}} \right)^2  
&  \geq 4+\frac{4}{b_{N-1}^2}  \frac{ \lambda_1}{n^2} \left([\hat{\vw}_{N-1}]_1 -[\hat{\vw}^{*}]_1 \right)^2
 \geq 4+   \frac{ 16}{ \eta^2 \lambda_1 } \left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2  \label{eq:b_n-1}
\end{align}
%\Rightarrow  \left( \frac{\eta \lambda_1^2}{ n b_{N-1}}  -2 \right) \left( \frac{\eta \lambda_1^2}{ n b_{N-1}}+2 \right)
%& \geq  \frac{ 16}{ \eta^2 \lambda_1^2 } \left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2\\
%\Rightarrow  \left( \frac{\eta \lambda_1^2}{ n b_{N-1}}  -2 \right) \left( \frac{\eta \lambda_1^2}{ n b_{N-1}}+2 \right)
%& \geq  \frac{ 16}{ \eta^2 \lambda_1^2 } \left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2\\
Thus we can further lower bound the term of the  summation in inequality  \eqref{eq:sum_term}  as follows
\begin{align}
\left( 1 - \frac{\eta \lambda_1}{ n b_{N-1}} \right)^{2} 
&= 1 + \frac{\eta \lambda_1}{ n b_{N-1}} \left(  \frac{\eta \lambda_1}{ n b_{N-1}} -2\right)   \nonumber\\
 & \geq  1 + \frac{\eta \lambda_1}{ n b_{N-1}} \left( \sqrt{4+   \frac{ 16}{ \eta^2 \lambda_1 } \left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2} -2 \right)    \text{ by inequality }\eqref{eq:b_n-1}    \nonumber\\
  & \geq  \sqrt{1+   \frac{ 4}{ \eta^2 \lambda_1 } \left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2}    \quad \text{ by inequality } b_{N-1}\leq \frac{\eta \lambda_1}{2n}    \nonumber
%    &=  1 + \frac{ \frac{ 4}{ \eta^2 \lambda_1 } \left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2}  { \sqrt{1+   \frac{ 4}{ \eta^2 \lambda_1 } \left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2} +1}   \nonumber
\end{align}
 Applying above inequality, we have the summation in  \eqref{eq:sum_term}  explicitly  lower bounded by
\begin{align}
\sum_{t=0}^{N-1}\left( 1 - \frac{\eta \lambda_1}{ n b_{N-1}} \right)^{2} 
& \geq 
\sum_{t=0}^{N-1}\left(1+   \frac{ 4}{ \eta^2 \lambda_1 } \left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2\right)^{t/2}   \nonumber\\
& \geq  \frac{  \eta^2\lambda_1}{4\left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2} \left(      \left(1+   \frac{ 4}{ \eta^2 \lambda_1 } \left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2\right)^{N/2}       -1\right) 
% \nonumber\\
%& \geq   \left(1+   \frac{ 4}{ \eta^2 \lambda_1 } \left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2\right)^{N/2}       +  \frac{  \eta^2\lambda^2_1}{4\left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2}  
\label{eq:summation}
\end{align}
Plugging above bound of summation \eqref{eq:summation} back to the \eqref{eq:sum_term}, we can estimate $N$:
\begin{align*}
N \leq 2 \log  \left(  1+
\frac{ \left({\eta \lambda_1} \right)^2 - 4(nb_0)^2 }{\eta^2 \lambda_1^2 }
\right) / \log \left (1+   \frac{ 4}{ \eta^2 \lambda_1 } \left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2 \right) 
\end{align*}
Replacing $\hat{\vw}_{0}=V^T\vw_0$ gives the bound  \eqref{eq:TheN1}.
%Even though $b_t \geq \frac{\eta \lambda_1}{2n}$ gives contraction for $\{\|\vw_t - \vw^*\|^2\}_{t>N}$. We need $b_t$ to be the greater than  $\frac{\eta( \lambda_1 +\lambda_n)}{2n}$ for faster convergence.  Let  $M$ be the first index such that  $b_{N+M+1}\geq \frac{\eta( \lambda_1 +\lambda_n)}{2n}$ from  $b_{N+M}<\frac{\eta( \lambda_1 +\lambda_n)}{2n}$. We now estimate the upper bound of $M$. Observe first that
%############################
%\begin{align*}
%%\left( \frac{\eta( \lambda_1+ \lambda_n) }{2n} \right)^2 \geq
%\frac{b_{t+1}^2}{ b_{t}^2}    \geq 1 + & \frac{ \lambda_1}{n^2 b_{t}^2} ([\hat{\vw}_{N+M-1}]_1  -[\hat{\vw}^{*}]_1  )^2 \\
%\Rightarrow  \frac{b_{N+M}^2}{ b_{N}^2} =\frac{b_{N+M}^2}{ b_{N+M-1}^2} \frac{b_{N+M-1}^2}{ b_{N+M-2}^2} \cdots  & \frac{b_{N+1}^2}{ b_{N}^2}  \geq  \prod_{t=N}^{M+N}  \left(1 +   \frac{ \lambda_1}{n^2 b_{t}^2} ([\hat{\vw}_{N+M-1}]_1 -[\hat{\vw}^{*}]_1 \right )^2
%% \\
%%\left( \frac{\eta( \lambda_1+ \lambda_n) }{2n} \right)^2 \geq b_{N+M}^2  & = b_{N+M-1}^2 +   \frac{ \lambda_1}{n^2} ([\hat{\vw}_{N+M-1}]_1 -[\hat{\vw}^{*}]_1  )^2 \\
%% \geq b_{0}^2 + \sum_{t=N}^{N+M}  \frac{ \lambda_1}{n^2} \left([\hat{\vw}_{t}]_1 -[\hat{\vw}^{*}]_1 \right)^2\notag
%%\\  
%%&= b_{0}^2 +  \frac{ \lambda_1}{n^2} \left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2 \sum_{t=M}^{N+M}  \left( 1 - \frac{\eta \lambda_1}{ nb_{t}} \right)^{2t}  \nonumber\\
%%&\geq b_{0}^2 +  \frac{ \lambda_1}{n^2} \left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2 \sum_{t=0}^{N-1}  \left( 1 - \frac{\eta \lambda_1}{ n b_{N-1}} \right)^{2t} 
%\end{align*}
%\begin{align}
%\left( \frac{\eta( \lambda_1+ \lambda_n) }{2n} \right)^2 \geq b_{N+M}^2  & \geq b_{N+M-1}^2 +   \frac{ \lambda_1}{n^2} ([\hat{\vw}_{N+M}]_1 -[\hat{\vw}^{*}]_1  )^2 \nonumber \\
%% \geq b_{0}^2 + \sum_{t=N}^{N+M}  \frac{ \lambda_1}{n^2} \left([\hat{\vw}_{t}]_1 -[\hat{\vw}^{*}]_1 \right)^2\notag
%%\\  
%&\geq b_{N+1}^2 +  \frac{ \lambda_1}{n^2} \sum_{t=N+1}^{N+M} \left([\hat{\vw}_{t}]_1 -[\hat{\vw}^{*}]_1 \right)^2 \nonumber\\
%&\geq \frac{\eta^2 \lambda_1^2}{4n^2} +  \frac{ \lambda_1}{n^2} \left([\hat{\vw}_{N}]_1 -[\hat{\vw}^{*}]_1 \right)^2 \sum_{t=1}^{M-1}  \prod_{\ell=0}^t  \left( 1 - \frac{\eta \lambda_1}{ n b_{\ell+N+1}} \right)^{2}\nonumber\\
%&\geq \frac{\eta^2 \lambda_1^2}{4n^2} +  \frac{ \lambda_1}{n^2} \left([\hat{\vw}_{N}]_1 -[\hat{\vw}^{*}]_1 \right)^2 \sum_{t=1}^{M-1} \left(\frac{\lambda_1-\lambda_n}{ \lambda_1+\lambda_n } \right)^{2t}
% \label{eq:lower3}
%\end{align}
%where  at the last inequality we use 
%\begin{align*}
%  \left( 1 - \frac{\eta \lambda_1}{ n b_{t+N+1}} \right)^{2}  &  \geq  \left(\frac{\lambda_1-\lambda_n}{ \lambda_1+\lambda_n } \right)^2, \quad \text{ for } b_{t+N+1}\in  \left(  \frac{\eta \lambda_1}{2n}, \frac{\eta( \lambda_1+\lambda_n)}{2n}\right).
% \end{align*}
%Since the geometric sum is
% \begin{align*}
% \sum_{t=1}^{M-1} \left(\frac{\lambda_1-\lambda_n}{ \lambda_1+\lambda_n } \right)^{2t}
% &=\frac{\left(\frac{\lambda_1-\lambda_n}{ \lambda_1+\lambda_n } \right)^2-\left(\frac{\lambda_1-\lambda_n}{ \lambda_1+\lambda_n } \right)^{2M}}{ 1- \left(\frac{\lambda_1-\lambda_n}{ \lambda_1+\lambda_n } \right)^{2}} = \frac{  }{}
% \end{align*}
% 
 
%which implies that to reach  $b_{N+1}\geq\frac{\eta \lambda_1}{2}$ we need the most steps is
%$$N =\bigg \lceil{ \log  \left(  1+
%\frac{ \left({\eta \lambda_1} \right)^2 - 4(nb_0)^2 }{\eta^2 \lambda_1^2 }
%\right) / \log \left (1+   \frac{ 4}{ \eta^2 \lambda_1 } \left([V^T\vw_{0}]_1 -[V^T\vw^{*}]_1 \right)^2 \right)\bigg \rceil} +1 $$
\end{proof}
Now we will prove the convergence for $b_t$ start from a very small initialization  $b_t\leq \eta \lambda_1/2n$
\begin{lem}
\label{lem:conv-small}\textbf{ (Linear Convergence Rate if  $b_0 < \frac{\eta\lambda_1}{ 2n}$)}
Under the same setup as Lemma \ref{lem:increase_sub}.  If $n b_0<\eta\lambda_1/2$,   we have $\| \vw_{T+s}-\vw^*\|^2\leq \epsilon$ for  the small constant $s$ satisfying
$$s \leq 2 \log  \left(  1+
\frac{ \left({\eta \lambda_1} \right)^2 - 4(nb_0)^2 }{\eta^2 \lambda_1^2 }
\right) / \log \left (1+   \frac{ 4}{ \eta^2 \lambda_1 } \left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2 \right) $$
and
\begin{align*}
T = &\max \left\{\widetilde{T}, \frac{\lambda_1}{\lambda_n}\left( 1+  \frac{ \| X \left( \vw_{0}-\vw^*\right)\|^2}{\eta^2 \lambda_1}+\log\left(\frac{ \eta \lambda_1}{2nb_0}\right) \right)\right\}\log\left(  \frac{\|\vw_{0}-\vw^*\|^2}{\lambda_n}+ \log\left(\frac{ \eta \lambda_1}{2nb_0}\right)\right) 
\end{align*}
where  $ \widetilde{T} := \max \left\{ \frac{\eta^2(\lambda_1+\lambda_n)^2 }{4\lambda_n} \frac{   n^2\left( \eta(\lambda_n+\lambda_1) /2+1 \right)}{  \lambda_1 \left(1-\frac{2\lambda_1}{(\lambda_1+\lambda_n) } \right)^2\left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2},   \frac{ (\lambda_1+\lambda_n )^2}{ 4 \lambda_1\lambda_n } \right\} $.
\end{lem}
\begin{proof}
Continuing with Lemma \ref{lem:increase_sub}, we have after $N$ steps such that
$b_{N+1}\geq \frac{\eta \lambda_1}{2n}$ and $b_{N}< \frac{\eta \lambda_1}{2n}$ from  $b_0 < \frac{\eta\lambda_1}{ 2n}$. Then we have contraction as in Lemma \ref{lem:conv-small}, for $t\geq N+1$
$$\| \vw_{t+1}-\vw^*\|^2
\leq\left( 1-\frac{2\eta \lambda_n}{nb_{t+1}} \left(1- \frac{\eta \lambda_1}{2nb_{t+1}}\right) \right)\| \vw_{t}-\vw^*\|^2.$$
Starting at $N+1$, we have $\|\vw_{N+1+T}-\vw^*\|\leq \epsilon$ by Lemma \ref{lem:conv-small}  where $T$ satisfies
\begin{align}
T = &\max \left\{\widetilde{T}, \frac{\lambda_1}{\lambda_n}\left( 1+  \frac{\| X \left(\vw_{N+1}-\vw^*\right)\|^2}{\lambda_1 \eta^2} \right)\right\}\log\left( \frac{\| \vw_{N+1}-\vw^*\|^2}{\epsilon}\right) \label{eq:fill-need}\\
\quad \text{where } \quad \widetilde{T} &:= \max \left\{ \frac{ (nb_{N+2})^2}{\lambda_n\left(2nb_{N+2}-\eta \lambda_1\right)} \mathbbm{1}_{ \left\{ b_{N+2}\in\left(\frac{ \eta \lambda_1}{2n}, \frac{ \eta( \lambda_1+\lambda_n) }{2n}\right) \right\} },   \frac{ (\lambda_1+\lambda_n )^2}{ 4 \lambda_1\lambda_n } \right\} \nonumber
\end{align}

where $b_{N+2} = \sqrt{b_{N+1}^2 + \frac{1}{n^2}\|X^TX(\vw_{N+1}-\vw^*)\|^2} >\frac{\eta \lambda_1}{2}$ assuming $\|X^TX(\vw_{N+1}-\vw^*)\|^2\neq0$.
However, we need to quantify  the convergence  rate in terms of the small initialization $b_0$ and $\| \vw_{0}-\vw^*\|^2$ instead of  $N$. That is, we need the following bounds
\begin{itemize}
\item[(a)] the upper bound for $ \|X(\vw_{N+1}-\vw^*)\|^2$  and $ \|\vw_{N+1}-\vw^*\|^2$;
\item [(b)] the upper bound for $\frac{ (nb_{N+2})^2}{\lambda_n\left(2nb_{N+2}-\eta \lambda_1\right)}$.
\item[(b)] the lower bound for $\left(b_{N+2}-\eta \lambda_1/(2n)\right)\mathbbm{1}{ \left\{ b_{N+2}\in\left( \frac{\eta \lambda_1}{2n} ,\frac{ \eta( \lambda_1+\lambda_n) }{2n}\right) \right\}   }$.
\end{itemize}

\paragraph{ (a) Upper bound for $ \|X(\vw_{N+1}-\vw^*)\|^2$  and $ \|\vw_{N+1}-\vw^*\|^2$  } We first estimate $ \|X(\vw_{N+1}-\vw^*)\|^2$ and  as in \cite{ward2018adagrad} and \cite{wu2018wngrad}.

 From \eqref{eq:ineq3}
\begin{align*}
\| X\left( \vw_{t+1}-\vw^*\right)\|^2
%&= \| X \left( \vw_{t}-\vw^*\right) -\frac{\eta}{b_{t+1}} X X^\top X \left( \vw_{t}-\vw^*\right) \|^2  \nonumber\\ 
%&\leq \| X \left( \vw_{t}-\vw^*\right)\|^2- \frac{2\eta}{nb_{t+1}} \left( 1 - \frac{\eta\lambda_1}{nb_{t+1}} \right)\| X^\top X \left(\vw_{t}-\vw^*\right)\|^2   \\
&\leq \| X \left( \vw_{t}-\vw^*\right)\|^2+ \frac{\eta^2\lambda_1}{n^2b_{t+1}^2} \| X^\top X \left(\vw_{t}-\vw^*\right)\|^2   \\
&\leq \| X \left( \vw_{0}-\vw^*\right)\|^2+ \sum_{\ell=0}^{t} \frac{\eta^2\lambda_1}{n^2b_{\ell+1}^2} \| X^\top X \left(\vw_{\ell}-\vw^*\right)\|^2   \\
&\leq \| X \left( \vw_{0}-\vw^*\right)\|^2+ \eta^2\lambda_1\log\left( b_{t+1}/b_0\right)  
\end{align*}
where in the last inequality we use Lemma \ref{lem:log-sum}.
Thus, we have  for $b_N<\frac{ \eta \lambda_1}{2n}$ and $b_{N+1}\geq\frac{ \eta \lambda_1}{2n}$
\begin{align}
\| X\left( \vw_{N+1}-\vw^*\right)\|^2\leq \| X\left( \vw_{N}-\vw^*\right)\|^2\leq  \| X \left( \vw_{0}-\vw^*\right)\|^2+ \eta^2\lambda_1\log\left(\frac{ \eta \lambda_1}{2nb_0}\right) \label{eq:lower-bound1}.
\end{align} 
We have from \eqref{eq:ineq2}
\begin{align}
\|  \vw_{t+1}-\vw^*\|^2
%&\leq \| \vw_{t}-\vw^*\|^2+ \frac{\eta^2}{n^2b_{t+1}^2} \|\vw_{t}-\vw^*\|^2  \nonumber \\
&\leq \|\vw_{0}-\vw^*\|^2+ \sum_{\ell=0}^{t} \frac{\eta^2}{n^2b_{\ell+1}^2} \| X^TX\left( \vw_{\ell}-\vw^*\right)\|^2  \nonumber  \\
&\leq \| \vw_{0}-\vw^*\|^2+ \sum_{\ell=0}^{t} \frac{\eta^2}{n^2b_{\ell+1}^2} \| X^TX\left( \vw_{\ell}-\vw^*\right)\|^2  \nonumber  \\
&\leq \|  \vw_{0}-\vw^*\|^2+ \eta^2\log\left( b_{t+1}/b_0\right)  \nonumber \\
\Rightarrow \|\vw_{N+1}-\vw^*\|^2&\leq \|\vw_{N}-\vw^*\|^2 \leq \| \vw_{0}-\vw^*\|^2+ \log\left(\frac{ \eta \lambda_1}{2nb_0}\right). \label{eq:lower-bound2}
\end{align}


\paragraph{(b) Lower bound for $\left(b_{N+2}-\eta \lambda_1/(2n)\right)\mathbbm{1}_{ \left\{ b_{N+2}\in\left( \frac{\eta \lambda_1}{2n} ,\frac{ \eta( \lambda_1+\lambda_n) }{2n}\right) \right\}   }$} We will estimate the lower bound of  $\left(b_{N+2}-\eta \lambda_1/(2n)\right)$ based on 
\begin{align}
\left(\frac{\eta \lambda_1}{2n} \right)^2\leq b_{N+1}^2
= &b_{N+2}^2- \frac{1}{n^2} \| X^\top X\left(\vw_{N+1}-\vw^* \right) \|^2  \label{eq:lower1} \\
\left([\hat{\vw}_{N+1}]_1-[\hat{\vw}^{*}]_1\right)^2 & = \left(1-\frac{\eta \lambda_1}{nb_{N+1} } \right)^2 ([\hat{\vw}_{N}]_1 -[\hat{\vw}^{*}]_1  )^2   \label{eq:lower2}
 \end{align}
%Note that for the value of $b_{N+2}$could  lays in:
%$$\text{either  }  \quad  b_{N+2}\geq \frac{\eta\lambda_1}{n} \quad  \text{ or} \quad  \frac{ \eta\lambda_1}{2n}<  b_{N+2}<  \frac{\eta\lambda_1}{n}.$$
%Suppose $\frac{ \eta\lambda_1}{2n}< b_{N+2}<  \frac{ \eta\lambda_1}{n} $.

%We first look at the extreme case: $\frac{ \eta\lambda_1}{2n} = b_{N+1} $. 
%Then inequality \eqref{eq:lower2} reduces to
%\begin{align}
%\left([\hat{\vw}_{N+1}]_1-[\hat{\vw}^{*}]_1\right)^2  =&([\hat{\vw}_{N}]_1 -[\hat{\vw}^{*}]_1  )^2 \geq ([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1  )^2 \label{eq:exteme}
%\end{align}
%Applying above equality \eqref{eq:exteme} and $b_{N+2}\in \left( \frac{\eta \lambda_1}{2n},\frac{\eta( \lambda_1+\lambda_n)}{2n}\right)$, we can get the lower bound from  \eqref{eq:lower1}
%\begin{align}
% \left( b_{N+2} - \frac{\eta \lambda_1}{2nb_{N+2}} \right)& \geq  \frac{ \frac{1}{n^2} \| X^\top X\left(\vw_{N+1}-\vw^* \right) \|^2}{\left( b_{N+2} +\frac{\eta \lambda_1}{2nb_{N+2}} \right)} 
%\geq \frac{  \lambda_1\left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2}{  n^2\left( \eta(\lambda_n+\lambda_1) /2+1 \right)} \label{eq:lower-bound2}.
%\end{align}
% thus we have 
%$\left(b_{N+2}-\eta \lambda_1/(2n)\right)$.
%But 
%\begin{align}
%\frac{ \| X^\top X\left(\vw_{N+1}-\vw^* \right) \|^2 }{n^2b^2_{N+2}}
%&= \frac{  \| X^\top X\left(\vw_{N+1}-\vw^* \right) \|^2 }{n^2b_{N+1}^2 + \| X^\top X\left(\vw_{N+1}-\vw^* \right) \|^2 } \nonumber\\
%%&\geq   \frac{  \lambda_1\left([\hat{\vw}_{N}]_1 -[\hat{\vw}^{*}]_1 \right)^2}{n^2b_{N+1}^2+  \lambda_1 \left([\hat{\vw}_{N}]_1 -[\hat{\vw}^{*}]_1 \right)^2 } \nonumber\\
%&\geq   \frac{  \lambda_1\left([\hat{\vw}_{N+1}]_1 -[\hat{\vw}^{*}]_1 \right)^2}{n^2b_{N+1}^2 +  \lambda_1 \left([\hat{\vw}_{N+1}]_1 -[\hat{\vw}^{*}]_1 \right)^2 } \nonumber\\
%&\geq   \frac{  \lambda_1\left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2}{ \eta \lambda_1 +  \lambda_1 \left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2 } 
%\end{align}
Note that $ \frac{\eta \lambda_1}{2n}\leq b_{N+1}\leq b_{N+2}<\frac{\eta( \lambda_1+\lambda_n)}{2n}$, we have  \eqref{eq:lower2} 
\begin{align}
\left([\hat{\vw}_{N+1}]_1-[\hat{\vw}^{*}]_1\right)^2 &  \geq  \left(\frac{\lambda_1-\lambda_n}{ \lambda_1+\lambda_n } \right)^2 ([\hat{\vw}_{N}]_1 -[\hat{\vw}^{*}]_1  )^2
 \end{align}
 Thus,  for $b_{N+2}\in \left( \frac{\eta \lambda_1}{2n},\frac{\eta( \lambda_1+\lambda_n)}{2n}\right)$
 \begin{align}
 \left( b_{N+2} - \frac{\eta \lambda_1}{2nb_{N+2}} \right)
 & \geq  \frac{ \frac{1}{n^2} \| X^\top X\left(\vw_{N+1}-\vw^* \right) \|^2}{\left( b_{N+2} +\frac{\eta \lambda_1}{2nb_{N+2}} \right)} \\
&\geq \frac{  \lambda_1 \left(\frac{\lambda_1-\lambda_n}{ \lambda_1+\lambda_n } \right)^2\left([\hat{\vw}_{0}]_1 -[\hat{\vw}^{*}]_1 \right)^2}{  \eta n(\lambda_n+\lambda_1) /2+n^2} \label{eq:lower-bound3}.
\end{align}
Putting the bounds \eqref{eq:lower-bound1} , \eqref{eq:lower-bound2} and \eqref{eq:lower-bound3} back to \eqref{eq:fill-need}, and adding the sharp estimate of $N$ from Lemma \ref{lem:increase_sub}, we get the statement. 
% thus we have
%\begin{align}
%\frac{ \| X^\top X\left(\vw_{N+1}-\vw^* \right) \|^2 }{n^2b^2_{N+2}}
%&= \frac{  \| X^\top X\left(\vw_{N+1}-\vw^* \right) \|^2 }{n^2b_{N+1}^2 + \| X^\top X\left(\vw_{N+1}-\vw^* \right) \|^2 } \nonumber\\
%%&\geq   \frac{  \lambda_1\left([\hat{\vw}_{N}]_1 -[\hat{\vw}^{*}]_1 \right)^2}{n^2b_{N+1}^2+  \lambda_1 \left([\hat{\vw}_{N}]_1 -[\hat{\vw}^{*}]_1 \right)^2 } \nonumber\\
%&\geq   \frac{  \lambda_1\left([\hat{\vw}_{N+1}]_1 -[\hat{\vw}^{*}]_1 \right)^2}{n^2b_{N+1}^2 +  \lambda_1 \left([\hat{\vw}_{N+1}]_1 -[\hat{\vw}^{*}]_1 \right)^2 } \nonumber\\
%&= \frac{  \lambda_1\left( 1 - \frac{\eta \lambda_1}{nb_{N}} \right)^2([\hat{\vw}_{N}]_1 -[\hat{\vw}^{*}]_1 )^2}{n^2b_{N+1}^2 +  \lambda_1 \left( 1 - \frac{\eta \lambda_1}{nb_{N+1}} \right)^2([\hat{\vw}_{N}]_1 -[\hat{\vw}^{*}]_1 )^2 } 
%\label{eq:lowerbound}
%\end{align}
%where the last equality is due to \eqref{eq:lower2}. Since 
%\begin{align*}
%\frac{b_{N+1}^2}{ \left( \frac{\eta \lambda_1}{nb_{N+1}}-1 \right)^2} 
%& = \frac{  \left(  b_{N}^2+ \| X^\top X\left(\vw_{N}-\vw^* \right) \|^2/n^2\right)^2 } {  \left(\eta \lambda_1- \sqrt{b_N^2+\| X^\top X\left(\vw_{N}-\vw^* \right) \|^2/n^2 } \right)^2} \\
%& \leq \frac{  \left(   \left(\frac{\eta \lambda_1}{2n} \right)^2 + \| X^\top X\left(\vw_{N}-\vw^* \right) \|^2/n^2\right)^2 } {  \left(\eta \lambda_1- \sqrt{\left( \frac{\eta \lambda_1}{2n} \right)^2+\| X^\top X\left(\vw_{N}-\vw^* \right) \|^2/n^2 } \right)^2}
%\end{align*} 
\end{proof}


\subsection{Proof of Theorem \ref{thm:fast}}
Now we give the proof of Theorem \ref{thm:fast}. According to the algorithm, we have
\begin{align}
s_{t+1}^{(i)} :=\left([V^T\vw_{t+1}]_i-[V^T{\vw}^{*}]_i\right)^2  =&\left( 1 - \frac{\eta \lambda_i}{nb_{t+1}} \right)^2([V^T{\vw}_{t}]_i -[V^T{\vw}^{*}]_i  )^2 
\end{align}




==> numeric_adagrad.tex <==
In this section, we use synthetic data to perform numerical experiment to corroborate how the adaptive stepsize robust is  to the choice of the parameters.


\begin{figure}[ht!!!!!]
%\minipage{0.8\textwidth}
\centering
  \includegraphics[width=\linewidth]{figs/iid}
%\endminipage\hfill
\caption{Standard Gaussian i.i.d. with size of training samples $n=500$  and dimension $d=1000$. Hidden layer has nodes $m=600$. $y\in \mathbb{R}^{500}$ is simulated by  standard Gaussian i.i.d.. Observe that $\max_{k} \|\vH(k)\|_2 \leq 1.4$ and $\min_{k} \lambda_{min}\left(\vH(k)\right) \ge 0.4$}
%\end{figure} 
% \begin{figure}[ht!!!!!]
%\minipage{0.8\textwidth}
\centering
  \includegraphics[width=\linewidth]{figs/corr}
%\endminipage\hfill
\caption{Gaussian Correlated (model same as Figure 1).  Observe that $\max_{k} \|\vH(k)\|_2 \leq 63$ and $\min_{k} \lambda_{min}\left(\vH(k)\right) \ge 0.017$ }
\end{figure}

We use synthetic data to illustrate the maximum  and minimum eigenvalues of $\mat{H} (k)$ for each iteration.  Figure 1 uses training dataset with each element follows i.i.d. standard Gaussian, we can see that the largest maximum eigenvalue is around $1.3$ and minimum eigenvalues is around $0.04$ within 100-epoch training. To some extent, it illustrates the cases between  general and best case where each sample are highly uncorrelated.  Figure 2 uses training dataset  follows multivariate Gaussian,we can see that the largest maximum eigenvalue is around $63$ and minimum eigenvalues is around $0.01$ within 100-epoch training.  To some extent, it illustrates the cases between  general and worse case where each sample are highly correlated with no zero mean.
 


==> proof_adagrad.tex <==
%\simon{Suggestion on proof structure:
%\begin{itemize}
%	\item A subsection just proving $\frac{b_0}{\eta} \ge C \norm{\mat{H}^\infty}$. Use induction as the current form and bound on $b_\infty$.
%	\item A subsection for $\frac{b_0}{\eta} \ge C \norm{\mat{H}^\infty}$. Use the same induction, add bounds on $T_0$ and $b_\infty$.
%\end{itemize}	
%	}
%
%

 In the following section, we give the detailed proof for Theorem \ref{thm:main_adagradloss}.
The proofs are organized into two parts. \textbf{Part I} in Subsection \ref{part1} is to prove the convergence for the initialization  $b_0/\eta \geq C \|\vH^{\infty}\|$. \textbf{Part II} in Subsection \ref{part2}  is to prove the convergence for the initialization  $b_0/\eta< C \|\vH^{\infty}\|$.   Several key lemmas will be stated and used during the proof,  and the proof of these lemmas will be deferred to subsection \ref{part3}. 

\subsection{Part I: Induction Proof of Theorem \ref{thm:main_adagradloss}}
\label{part1}
In this part, we  prove the following condition by induction: \emph{show Condition~\ref{con:adagrad_sub} for every $k =0,1,2\ldots$. Based on this condition, we then obtain the upper bound of $b_k$ and so the convergence result.}\\
%\textbf{Condition \ref{con:adagrad_sub}}
%At the $k$-th iteration,  
%\begin{align}
% \norm{\vy-\vu(k)}^2 
%   &\leq \left(  1- \frac{\eta  \lambda_0 C_1}{b_{k}}\left(1-\frac{\eta C{\|\vH^\infty\|}}{b_{k}} \right) \right)\norm{\vect{y}-\vect{u}(k-1)}^2 
%\label{eq:main_adagrad1}
%\end{align} 
%where we define 
%$\norm{\vect{y}-\vect{u}(-1)}^2 =\norm{\vect{y}-\vect{u}(0)}^2  /\left(1- \frac{\eta  \lambda_0 C_1}{b_{0}}\left(1-\frac{\eta C{\|\vH^\infty\|}}{b_{0}} \right) \right) $,   $C_1$ and $C$ are some constant  of order $1$ (see Table \ref{table}  in Appendix \ref{sec:basic} for details).


For the base case $k'=0$, by definition Condition~\ref{con:adagrad_sub} holds. Suppose for $k'=0,\ldots,k$, Condition~\ref{con:adagrad_sub} holds, and we want to show it still holds for $k'=k+1$. We first prove the  order of $m$ and then the contraction of $\norm{\vect{u}(k+1)-\vect{y}}$.


For the order of $m$ that controls the strict positiveness of $\{\vH(k')\}_{k'=0}^k$ and so the contraction of $\norm{\vect{u}(k+1)-\vect{y}}$, \footnote{For more descriptions of the relationship between $m$ and $\norm{\vect{u}(k+T_0)-\vect{y}}$, we refer to Subsection \ref{sec:order_m_gd}} we  first have that $m = \Omega\left(\frac{n^2}{\lambda_0^2} \log^2\left(\frac{n}{\delta}\right)\right)$  from Lemma \ref{lem:H0_close_Hinft}. 
Further, by Lemma \ref{lem: small_w_for_allbsq_sub} with $T_0=1$ for the adaptive stepsize $b_{k'}\geq \eta C\|\vH^{\infty}\|$ , we can upper bound $\|\vw_r(k+1)-\vw_r(0)\|$ by  $ \widetilde{R}$. By Lemma \ref{lem:close_to_init_small_perturbation}, we ask for $\widetilde{R}\leq R$ for $k'=0,1,\cdots, k+1$, which results in  $m = \Omega(\frac{n^6}{\lambda_0^4\delta^3}). $ \\ 
\textbf{Lemma \ref{lem: small_w_for_allbsq_sub}}
Suppose Condition~\ref{con:adagrad_sub} holds for $k'=0,\ldots,k$ and  $ b_k$ is updated by Algorithm 1. Let  $T_0\geq 1$ be the first index such that $b_{T_0} \geq  \eta C \|\vH^{\infty}\|$. Then for every $r \in [m]$, we have for $k = 0,1,\cdots,$
\begin{align*}
 & b_{k}\leq b_{T_0}+\frac{4\alpha^2 \sqrt{n}}{\eta {\lambda_0}C_1}\norm{\vy-\vu(T_0-1)};\\
\|\vw_r(k+T_0)-&\vw_r(T_0-1)\| 
\leq \frac{4 \sqrt{n} }{\sqrt{m} \lambda_0 C_1} 
 \norm{\vy-\vu(T_0-1)} \triangleq \widetilde{R}.
\end{align*}

Now, given the strict positiveness of $\{\vH(k')\}_{k'=0}^k$ such that $\lambda_{min}\left( \vH(k')\right)>\frac{\lambda_0}{2}$, we will prove \eqref{eq:main_adagrad1} at iteration $k+1$. We follow the same argument as Subsection  \ref{sec:contraction_gd} and straightforwardly modify the constant learning rate $\eta$ for the adaptive learning rate $\eta/b_{k+1}$. Observe the key inequality \eqref{eq:keyforadagrad} in Subsection  \ref{sec:contraction_gd} that  expresses the gradient descent with constant learning rate $\eta$ in Theorem \ref{thm:main_gd}, and we have,
\begin{align}
 \norm{\vy-\vu(k+1)}^2 
   &\leq \left(  1- \frac{\eta  \lambda_0 C_1}{b_{k+1}}\left(1-\frac{\eta}{b_{k+1}} C_{\|\vH(0)\|}\right) \right)\norm{\vect{y}-\vect{u}(k)}^2 
  \label{eq:LipchitzFuc}
\end{align} 
which is Condition \ref{con:adagrad_sub} for $k'=k+1$.

Now that we have proved Condition \ref{con:adagrad_sub} for all $k=0,1,2,\cdots,$ when $b_0/\eta \geq C\|\vH^{\infty} \|$. We use  Lemma \ref{lem: small_w_for_allbsq_sub} again to bound $b_k$ denoted by $b_{\infty}$:
$$b_{\infty} \leq  b_{0}+\frac{4\alpha^2 \sqrt{n}}{\eta {\lambda_0}C_1}\norm{\vy-\vu(0)}=O\left(b_{0}+\frac{\alpha^2 n}{\eta \lambda_0 \delta}  \right) $$
where the equality is from Proposition \ref{prop:a2}. 
%\begin{lem}
%\label{lem:bupper}
%Suppose Condition~\ref{con:adagrad} holds for $k'=0,\ldots,k$ and  $ b_k$  updated by Algorithm 1 . Let  $T_0\geq 1$ be the first index such that $b_{T_0} /\eta \geq  C \|\vH^{\infty}\|$. Then $b_k$ is bounded by 
%\begin{align*}
%b_{k}  \leq b_{T_0}+\frac{2\alpha^2 \sqrt{n}}{\eta {\lambda_0}C_1}\norm{\vy-\vu(T_0-1)},\quad  k = 0,1,\cdots.
%\end{align*}
%\end{lem} 
Thus, iteratively substituting  $ \norm{\vy-\vu(t)}^2, t = k-1, k-1, \cdots, 0$  in inequality \eqref{eq:LipchitzFuc}, we have
\begin{align}
 \norm{\vy-\vu(T)}^2 
  &\leq \Pi_{t=0}^{T-1}\left( 1-\frac{\eta \lambda_0C_1}{2 b_{t}}\right)\norm{\vy-\vu(0)}^2
%  &\leq \exp\left( - \sum_{t=0}^{T-1}\frac{\eta \lambda_0C_1}{2b_{t}} \right)\norm{\vy-\vu(0)}^2 \nonumber\\
  \leq \exp\left( -T \frac{\eta \lambda_0C_1}{2b_{\infty}}  \right)\norm{\vy-\vu(0)}^2 \nonumber.
\end{align}
For tolerance error $\varepsilon$ such that $ \norm{\vy-\vu(T)}^2 \leq \varepsilon$, we get the maximum step by plugging the upper bound $b_{\infty}$ into the above inequality.

%Since $\{b_{t}\}_{t=0}^{k+1}$ is a monotone sequence, we have $b_{k+T_0}\geq b_{k+T_0-1}\geq b_{T_0} \geq L = \max\{1, 2\eta C_{\| \mat{H}(0)\|} \}$, thus  inequality \eqref{eq:LipchitzFuc} can be further reduced to
%\begin{align*}
% \norm{\vy-\vu(k+T_0)}^2 
%   &\leq \left(  1- \frac{\eta \lambda_0 C_1}{2b_{k+T_0}} \right)\norm{\vect{y}-\vect{u}(k+T_0-1)}^2  \\
%      &\leq \left(  1- \frac{\eta \lambda_0 C_1}{2b_{k+T_0}} \right) \Pi_{t=0}^{k-1}(1-\frac{\eta \lambda_0}{2b_{t+T_0}})\norm{\vy-\vu(T_0-1)}^2 \\
%           &\leq  \Pi_{t=0}^{k}(1-\frac{\eta \lambda_0}{2b_{t+T_0}})\norm{\vy-\vu(T_0-1)}^2 
%\end{align*} 





\subsection{Part II: Induction Proof of Theorem \ref{thm:main_adagradloss}}
\label{part2}

Starting with $ b_0/\eta < C\|\vH^{\infty} \|$, we  use Lemma \ref{lem:increase_sub} 
with $\gamma = \alpha^2 \sqrt{n} $,  $a_j = \|\vy-\vu(k)\|  $ and $L = \left( \eta C\|\vH^{\infty} \| \right)^2$
 to prove that eventually after step 
\begin{align}
T_0=\bigg \lceil{ \frac{\left(\eta C\|\vH^{\infty} \|\right)^2 -b_0^2 }{\alpha^2 \sqrt{ n \varepsilon} }  \bigg \rceil} +1,
\label{eq:T0}
\end{align}
we have
\begin{align}
\text{either } \quad \min_{t\in [T_0]} \|\vy-\vu(t)\|^2 \leq  \varepsilon, \quad  \text{or}\quad  \quad b_{T_0} \ge  \eta C\|\vH^{\infty} \| .
\label{eq:twocond}
\end{align}
%\textbf{Lemma \ref{lem:increase_sub}}
%Fix $\varepsilon \in (0,1]$, $L > 0$, $\gamma>0$.   For any non-negative $a_0, a_1, \dots, $ the dynamical system
%$$
%b_0 > 0; \quad  \quad b_{j+1}^2 = b_j^2 +  \gamma a_j
%$$
%has the property that after 
%{$N = \lceil{ \frac{ L^2-b_0^2}{ \gamma\sqrt{\varepsilon}} \rceil}+1$}
%iterations, either $\min_{k=0:N-1}  a_k  \leq  \sqrt{\varepsilon}$, or $b_{N} \geq  L$. 

\emph{Now, similar to \textbf{ Part I}, we  first use induction to prove Condition \ref{con:adagrad_sub} with $m$ satisfying 
\begin{align}
m&=\Omega \left ( \frac{4 n^{5} }{\lambda_0^4\delta^2 }  
 \left(  2\norm{\vy-\vu(0)}^2 + \frac{ \eta^4C^2 \lambda_0 \|\vH^\infty\|^2  \left(4\sqrt{C\|\vH^\infty\|} + \lambda_0\right)^2}{ 2\alpha^4n } \right)\right) . 
\label{eq:m_large}
\end{align}
Note that since $T_0> 1$,  we will first prove the induction before $k\leq T_0-1$ and then  $k\geq T_0$. Based on this condition, we then obtain the upper bound of $b_k$ and so the convergence result.}

 For  $k'=0$, by definition Condition~\ref{con:adagrad_sub} holds. Suppose for $k'= 0, 1,\ldots, k \leq T_0-2$ , Condition~\ref{con:adagrad_sub} holds, and we want to show it  holds for $k'=k+1 \leq T_0-1$. 
 Similar to \textbf{Part I}, we use Lemma \ref{lem:close_to_init_small_perturbation} in order to maintain the strict positiveness of $\vH(k
 )$  for $k'=k+1 \leq T_0-1$. That is,   we ask for $k'=0,1,\cdots, k+1$ such that  $ \|\vw_r(k')-\vw_r(0)\|\leq R= \frac{c\lambda_0 \delta}{n^2}$.  From Lemma~\ref{lem: small_w_for_allbsq1_sub}, we know that the upper bound of the distance $\|\vw_r(t)-\vw_r(0)\|$ for $t\leq T_0-1$ grows only up to a finite number  proportional to $ \eta C \| \vH^{\infty}\|$.
\\
\textbf{Lemma \ref{lem: small_w_for_allbsq1_sub}}
Let $L = \eta C \|\vH^{\infty}\|$  and $T_0\geq 1$ be the first index such that $b_{T_0} \geq  L $. Then for every $r \in [m]$, we have $k\leq T_0-2$
\begin{align*}
\|\vw_r(k+1)-\vw_r(0)\|
&\leq 
 \frac{2\eta^2 C\|\vH^{\infty}\|}{ \alpha^2\sqrt{ m}} \triangleq \hat{R}.
\end{align*}

Thus, we have  the strict positiveness of $\{\vH(k')\}_{k'=0}^k,, k \leq T_0-1$ such that $\lambda_{min}\left( \vH(k')\right)>\frac{\lambda_0}{2}$, as long as $ \hat{R}\leq \frac{c\lambda_0 \delta}{n^2}$ holds. But that is guaranteed for large $m$ satisfying \eqref{eq:m_large}.
Again, use the same argument as the derivation of inequality \eqref{eq:LipchitzFuc}, we have Condition \ref{con:adagrad_sub} holds for $k'=k+1$.
Thus, we prove Condition \ref{con:adagrad_sub} for $k'=0,1,\ldots, T_0-1$.  


Now we are at $k' = T_0$. We have no clue at iteration $k'=T_0$ since there is no contraction bound  for  $\norm{\vy-\vu(k')}^2$,  $k'=0,1, k \leq T_0-1$. However, we have \eqref{eq:twocond} at $k'=T_0$. 

If we are lucky to have $$ \min_{t\in [T_0]} \|\vy-\vu(t)\|^2 \leq  \varepsilon,$$ then we are done. Otherwise, we have $b_{T_0}\geq \eta C\|\vH^\infty\|$. We will continue to prove the Condition \ref{con:adagrad_sub} for $k'=T_0, T_0+1,\ldots$. 

For the case $k'=T_0$, we need to prove the  strictly positive $\vH(T_0)$ given  Condition \ref{con:adagrad_sub} holds for $k'= 0, 1, \ldots, T_0-1$. At this time,  the upper bound of $ \norm{\vy-\vu(T_0-1)}  $ only grows up to a  factor  of $\eta C\|\vH^{\infty}\|$ as stated in the following lemma,

\textbf{Lemma \ref{lem:log_growth_sub}}
Let $T_0\geq 1$ be the first index such that $b_{T_0} \geq  \eta C \|\vH^{\infty}\| $. Suppose Condition \ref{con:adagrad_sub} holds for $k=0,1,\ldots,k$. Then
\begin{align*}
\norm{\vy-\vu(T_0-1)}
 \leq & \norm{\vy-\vu(0)} +  \frac{ 2\eta^2 \sqrt{\lambda_0} \left(C\|\vH^\infty\|\right)^{3/2}}{   \alpha^2\sqrt{n}}.
\end{align*}

Then the distance between $\vw_r(T_0)$ and $\vw_r(0)$  is
\begin{align*}
\|\vw_r(T_0)-\vw_r(0)\|
&\leq \|\vw_r(T_0)-\vw_r(T_0-1)\|+ \|\vw_r(T_0-1)-\vw_r(0)\| \nonumber\\
&\leq  \frac{\eta}{b_{T_0}} \norm{\frac{\partial L(\vW{(T_0-1)})}{\partial \vw_r}} + \frac{2\eta^2 C\|\vH^{\infty}\|}{ \alpha^2\sqrt{ m}} \nonumber\\
&\leq  \frac{ \sqrt{n} \|\vy-\vu(T_0-1)\| }{C\|\vH^{\infty} \| \sqrt{m}}  + \frac{2\eta^2 C\|\vH^{\infty}\|}{ \alpha^2\sqrt{ m}} \\
&\leq  \frac{1}{\sqrt{m}} \left(  \frac{ \sqrt{n} \|\vy-\vu(0)\| }{C\|\vH^{\infty} \| }  + \frac{\eta^2}{ \alpha^2} \left(  \sqrt{\lambda_0 C\|\vH^{\infty}\| }+ C\|\vH^{\infty}\|\right)  \right)\\
&\leq   \frac{c\lambda_0\delta}{n^2}
\end{align*}
where the last inequality is due to large $m$ satisfying equation \eqref{eq:m_large}. Thus, Lemma \ref{lem:close_to_init_small_perturbation}  implies the  strict positives for $\vH(T_0)$ such that $\lambda_{min}(\vH(T_0))\geq \frac{\lambda_0}{2}>0$ and so Condition \ref{con:adagrad_sub} holds for $k=T_0$.
%since the lower bound of $b_{T_0-1}$ is 
%\begin{align*}
%b_{T_0-1} &= b_{T_0-2} +\frac{ \alpha^2 \sqrt{n}\norm{\vy-\vu(T_0-2)} }{b_{T_0-1}+ b_{T_0-2}}\\
%&\geq  b_{T_0-2} +\frac{ \alpha^2 \sqrt{n}\norm{\vy-\vu(T_0-1)} }{2b_{T_0-1}} \\
%&\geq  b_{0} +\sum_{t=0}^{T_0-1} \frac{ \alpha^2 \sqrt{n}\norm{\vy-\vu(T_0-1)} }{2b_{T_0-1}}
%\end{align*}

Now suppose for $k'= 0,\ldots, T_0-1, T_0,\ldots,k+T_0-1,$  Condition~\ref{con:adagrad_sub} holds, and we want to show it holds for $k'=k+T_0$. The bound $\|\vw_r(k+T_0)-\vw_r(0)\|$  can be obtained by using Lemma \ref{lem: small_w_for_allbsq_sub}, Lemma \ref{lem: small_w_for_allbsq1_sub}
\begin{align}
\|\vw_r(k+T_0)-\vw_r(0)\|
&\leq \|\vw_r(k+T_0)-\vw_r(T_0-1)\|+ \|\vw_r(T_0-1)-\vw_r(0)\| \nonumber\\
&\leq  \frac{4 \sqrt{n} }{\sqrt{m} \lambda_0 C_1} \left( 
\norm{\vy-\vu(T_0-1)} + \frac{ \eta^2 \lambda_0 C\|\vH^{\infty}\|}{ 2\alpha^2 \sqrt{n}} \right)
 .\label{eq:mLa}
\end{align}
Putting back the upper bound of $\norm{\vy-\vu(T_0-1)}$ given in Lemma \ref{lem:log_growth_sub} and using Lemma \ref{lem:close_to_init_small_perturbation} that ask for $ \|\vw_r(k+T_0)-\vw_r(0)\|\leq R= \frac{c\lambda_0 \delta}{n^2}$, we require following
\begin{align*}
 \frac{c\lambda_0 \delta}{n^2} &\geq   \frac{4 \sqrt{n} }{\sqrt{m} \lambda_0 C_1} \left(  \norm{\vy-\vu(0)} + \frac{ \eta^2 C\|\vH^\infty\| \sqrt{ \lambda_0}  \left(4 \sqrt{C\|\vH^\infty\|} + \sqrt{\lambda_0}\right)}{ 2\alpha^2 \sqrt{n}} \right).
\end{align*}
Rearranging  $m$ to one side, we get \eqref{eq:m_large}.
Given the strictly positive $\{\vH(k')\}_{k'=0}^{k+T_0}$,  we have Condition \ref{con:adagrad_sub} holds for $k'=k+T_0$ by the same argument as the derivation of  inequality \eqref{eq:LipchitzFuc}. Thus, we prove Condition \ref{con:adagrad_sub} for $k'=T_0,T_0+1,\ldots$.  



Now that we prove  Condition \ref{con:adagrad_sub} for $k'=0, \ldots,T_0-1, T_0,T_0+1,\ldots$,  we use Lemma \ref{lem: small_w_for_allbsq_sub} and Lemma \ref{lem:log_growth_sub}  to bound $b_k$ denoted by $\bar{b}_{\infty}$:
\begin{align}
\bar{b}_\infty = \eta C\|\vH^{\infty}\|+\frac{4\alpha^2 \sqrt{n}}{\eta {\lambda_0}C_1}\left( \norm{\vy-\vu(0)} + \frac{ 2\eta^2 \sqrt{\lambda_0}   \left(C\|\vH^\infty\| \right)^{3/2}}{ \alpha^2 \sqrt{n}  } \right)
\end{align}
Thus, using the fact that $b_{T_0}/\eta \geq C\|\vH^{\infty}\|$ with $T_0=\frac{\left(\eta C\|\vH^{\infty} \|\right)^2 -b_0^2 }{\alpha^2 \sqrt{ n\varepsilon} }$ and iteratively substituting  $ \norm{\vy-\vu(t)}^2$, $t = T-1,T-2, \cdots, T_0-1 $  in inequality \eqref{eq:LipchitzFuc} gives
\begin{align}
 \norm{\vy-\vu(T)}^2 
  &\leq \Pi_{t=T_0}^{T}\left( 1-\frac{\eta \lambda_0C_1}{2 b_{t}}\right)\norm{\vy-\vu(T_0-1)}^2 \nonumber \\
  &\leq \exp\left( - (T-T_0+1) \frac{\eta \lambda_0C_1}{2\bar{b}_\infty}  \right) \left(  \norm{\vy-\vu(0)} +    \frac{ 2\eta^2  \left(C\|\vH^\infty\| \right)^{3/2}}{ \alpha^2 \sqrt{\lambda_0} } 	\right)^2. \nonumber
\end{align}
For the tolerance $\varepsilon$, the maximum step $T$ can be derived by plugging the upper bound $\bar{b}_{\infty}$ into the above inequality.

%\subsection{Proof of Lemmas}

 \subsection{Ingredients of Proof of Theorem \ref{thm:main_adagradloss}}
 We will  be using the following key  inequalities for $\vH^\infty$ giving the over-parameterization $m$ sufficiently large such that at $t$ iteration $\vH(t)$ is strictly positive:
%\begin{align}
%\|\vu(t+1)-\vy\|^2
%&\leq \left( 1-\frac{2\eta \lambda_0}{b_{t+1}} \left(1- \frac{\eta \|\vH^\infty\|}{2b_{t+1}}\right) \right)\|\vu(t)-\vy\|^2\label{eq:ineq2} \\
%\|\vu(t+1)-\vy\|^2
%&\leq  \left( 1- \frac{2\eta \|\vH^\infty\|  \lambda_0}{ ( \lambda_0+\|\vH^\infty\|)b_{t+1}}\right)\|\vy-\vu(t)\|^2 \nonumber\\
%&\quad  +\frac{\eta}{b_{t+1}} \left(\frac{\eta}{b_{t+1}}- \frac{2}{ \lambda_0 +\|\vH^\infty\|}\right)\|\vH^\infty \left(\vy-\vu(t)\right)\|^2   \label{eq:ineq3}\\
%\| (\vH^\infty )^{1/2}\left(\vu(t+1)-\vy\right)\|^2
%&\leq \left(1- \frac{2\eta}{b_{t+1}} \left( 1 - \frac{\eta\|\vH^\infty\|}{2b_{t+1}} \right) \right)\| \vH^\infty \left(\vy-\vu(t)\right)\|^2   \label{eq:ineq1}
%\end{align}
 
\label{subsec:ingredients}
\label{part3}
%As we have seen in the proof sketch. 
%Lemma~\ref{lem: small_w_for_allbsq_sub} and Lemma~\ref{lem: small_w_for_allbsq1_sub} are most important lemmas in the proof of Theorem~\ref{thm:main_adagradloss}.
%Here we state and prove these two lemmas.
 \begin{lem}
\label{lem: small_w_for_allbsq_sub}
Suppose Condition~\ref{con:adagrad_sub} holds for $k'=0,\ldots,k$ and   $ b_k$  is updated by Algorithm 1. Let $T_0\geq 1$ be the first index such that $b_{T_0} \geq  \eta C \|\vH^{\infty}\| $.  Then for every $r \in [m]$ and $k = 0,1,\cdots$,
\begin{align*}
 & b_{k}\leq b_{T_0-1}+\frac{4\alpha^2 \sqrt{n}}{\eta {\lambda_0}C_1}\norm{\vy-\vu(T_0-1)} ;\\
\|\vw_r(k+T_0)-&\vw_r(T_0-1)\| 
\leq \frac{4 \sqrt{n} }{\sqrt{m} \lambda_0 C_1} 
 \norm{\vy-\vu(T_0-1)}  \triangleq \widetilde{R} .
\end{align*}
\end{lem} 


\textbf{Proof of Lemma \ref{lem: small_w_for_allbsq_sub}}
When $b_{T_0}/\eta \geq \frac{C \|\vH^{\infty}\|}{2}$ at some $T_0\geq 1$, thanks to the key fact that Condition~\ref{con:adagrad_sub} holds $k'=0,\ldots,k$, we have
\begin{align*}
\norm{\vy-\vu(k+T_0)}^2
\leq & {\left( 1-\frac{\eta \lambda_0}{2b_{k+T_0})} \right)} \norm{\vy-\vu(k+T_0-1)} ^2\\
 \leq  &\left( 1-\frac{\eta \lambda_0 C_1}{4b_{k+T_0}} \right) \norm{\vy-\vu(k+T_0-1)} ^2 \\
 \leq & \norm{\vy-\vu(T_0-1)}^2-\sum_{t=0}^{k}\frac{\eta \lambda_0 C_1}{4b_{t+T_0}}\norm{\vy-\vu(t+T_0-1)}^2 \\
 \Rightarrow  \quad \sum_{t=0}^{k} &\frac{\norm{\vy-\vu(t+T_0-1)}^2}{b_{t+T_0}} \leq  \frac{4 \norm{\vy-\vu(T_0-1)}   }{\eta \lambda_0 C_1}^2.
 \end{align*}
Thus, the upper bound for $b_k$,
\begin{align*}
b_{k+T_0} 
%=  & b_{k+T_0-1}  +\frac{\alpha^2\sqrt{m}}{b_{k+T_0}+b_{k+T_0-1}} \max_{r\in[m]}\norm{\frac{\partial L(\vW(k+T_0-1))}{\partial\vw_r}}_{2}\\
\leq& b_{k+T_0-1}  + \frac{\alpha^2\sqrt {n} }{b_{k+T_0}} \|\vy - \vu(k+T_0-1)\| \\
\leq&b_{T_0-1} +\sum_{t=0}^{k}\frac{\alpha^2\sqrt {n} }{b_{t+T_0}} \|\vy - \vu(t+T_0-1)\| \\
\leq &b_{T_0-1} +\frac{4\alpha^2\sqrt {n} }{\eta {\lambda_0}C_1}\norm{\vy-\vu(T_0-1)}.
\end{align*}
As for the  upper bound of $\|\vw_r(k+T_0)-\vw_r(T_0-1)\|,$
\begin{align*}
 \|\vw_r(k+T_0)-\vw_r(T_0-1)\|
\leq& \sum_{t=0}^{k}\frac{\eta }{b_{t+T_0}} \| \frac{\partial L(\vW{(t+T_0-1)})}{\partial \vw_r } \| \\
%\leq & \frac{\eta \sqrt{n}}{\sqrt{m}}\sum_{t=0}^{k}\frac{1}{b_{t+T_0}} \| \vy - \vu(t+T_0-1)\| \\
 \leq& \frac{4 \sqrt{n} }{\sqrt{m} \lambda_0 C_1} \norm{\vy-\vu(T_0-1)}.  
\end{align*}



\begin{lem}
\label{lem: small_w_for_allbsq1_sub}
Let  $T_0\geq 1$ be the first index such that $b_{T_0} \geq  \eta C \|\vH^{\infty}\| $. Then for every $r \in [m]$, we have for $k=0,1,\ldots,T_0-1$,
\begin{align*}
\|\vw_r(k)-\vw_r(0)\|
\leq 
 \frac{4\eta^2C\|\vH^{\infty}\|}{ \alpha^2\sqrt{m}} \triangleq \hat{R}.
\end{align*}
\end{lem}






\textbf{Proof of Lemma \ref{lem: small_w_for_allbsq1_sub}}
For the upper bound of $\|\vw_r(k+1)-\vw_r(0)\|$ when $b_{t}/\eta < C \|\vH^{\infty}\|$, $t = 0,1, \cdots, k$ and $k\leq T_0-2$, we first
observe that
\begin{align*}
 \sum_{t=0}^{k}\frac{\norm{\vy-\vu(t)}}{b_{t+1}}  
 &\leq  \frac{1}{ \alpha^2 \sqrt{ n} }\sum_{t=0}^{k}   \frac{ \alpha^2 \sqrt{ n} \norm{\vy-\vu(t)} }{  \sqrt{ \alpha^2\sqrt{ n}\sum_{\ell=0}^{t} \| \vy-\vu(\ell)\|+b_0^2}} \nonumber \\
&\leq  \frac{2}{ \alpha^2 \sqrt{ n} }\sqrt{  \alpha^2\sqrt{ n}\sum_{\ell=0}^{k}\| \vy-\vu(\ell)\|+b_0^2} \nonumber \\
&\leq  \frac{ 2b_{T_0-1} }{ \alpha^2 \sqrt{ n} }
\end{align*}
where the  second inequality use Lemma \ref{lem:sqrtsum} and the third inequality is due to the fact that $b_k \leq b_{T_0-1} \leq \eta C \|\vH^{\infty}\|$ for all $k\leq T_0-2$.  Thus,
\begin{align*}
\|\vw_r(k+1)-\vw_r(0)\|   \leq& \sum_{t=0}^{k}\frac{\eta }{b_{t+1}} \| \frac{\partial L(\vW{(t)})}{\partial \vw_r } \| 
\leq  \frac{\eta \sqrt{n}}{\sqrt{m}}\sum_{t=1}^{k}\frac{ \| \vy - \vu(t)\|}{b_{t+1}} 
\leq  \frac{2C \eta^2 \|\vH^{\infty}\|}{ \alpha^2\sqrt{ m}}.
\end{align*}

%
%
%Proof of Lemma \ref{lem: small_w_for_allbsq_sub}  and \ref{lem: small_w_for_allbsq1_sub} are given in subection \ref{subsec:ingredients} \\
\begin{lem}
\label{lem:log_growth_sub}
Let $T_0\geq 1$ be the first index such that $b_{T_0} \geq  \eta C \|\vH^{\infty}\| $. Suppose Condition \ref{con:adagrad_sub} holds for $k=0,1,\ldots,k$. Then
\begin{align*}
\norm{\vy-\vu(T_0-1)}
 \leq & \norm{\vy-\vu(0)} +  \frac{ 2\eta^2 \sqrt{\lambda_0} \left(C\|\vH^\infty\|\right)^{3/2}}{   \alpha^2\sqrt{n}}.
\end{align*}
\end{lem}
\textbf{Proof of Lemma \ref{lem:log_growth_sub}}
\begin{align}
\norm{\vy-\vu(T_0-1)}  &\leq  \sqrt{ 1+\frac{\eta^2\lambda_0 C{\|\vH^\infty\|} }{b^2_{T_0-1}} }\norm{\vy-\vu(T_0-2)} \nonumber\\
&\leq  \norm{\vy-\vu(T_0-2)} +\frac{\eta \sqrt{ \lambda_0 C \|\vH^\infty\|} }{b_{T_0-1}} \norm{\vy-\vu(T_0-2)} \nonumber\\
 &\leq \norm{\vy-\vu(0)} + \frac{ \eta \sqrt{ \lambda_0 C \|\vH^\infty\|}}{ \alpha^2 \sqrt{n} } \sum_{t=0}^{T_0-2}  \frac{ \alpha^2 \sqrt{ n} \norm{\vy-\vu(t)} }{  \sqrt{ \alpha^2\sqrt{ n}\sum_{\ell=0}^{t} \| \vy-\vu(\ell)\|+b_0^2}}  \nonumber\\
    &\leq \norm{\vy-\vu(0)} +   \frac{ 2\eta \sqrt{\lambda_0 C \|\vH^\infty\|}}{ \alpha^2  \sqrt{n} } \sqrt{ \alpha^2\sqrt{ n}  \sum_{\ell=0}^{T_0-2} \| \vy-\vu(\ell)\|+b_0^2} \nonumber \\
        &\leq \norm{\vy-\vu(0)} +  \frac{ 2\eta^2 \sqrt{\lambda_0} \left(C\|\vH^\infty\| \right)^{3/2}}{ \alpha^2  \sqrt{n}}  \nonumber
\end{align}               

   

==> rebuttal-sgd.tex <==
\subsection{With learning rate smaller than $\frac{\lambda_0}{n}$ } 
\begin{lem}
For $t = 0,1,\ldots, T-1$, let
$$Z_{t} =\log(\norm{\vect{y}-\vect{u}(t)}^2) - t\log\left(1-\frac{\eta \lambda_0}{2n}\right),$$ then Then $Z_{t}$ is a super-martingale. Furthermore, we have with probability $1-\exp()$ such that 

\end{lem}
\begin{proof}

Observe from inequality \eqref{eq:y-u1} and use $\log(1+x)\leq x$ that  $\forall t\in[T]$
\begin{align*}
   \mathbb{E}\left[Z_{t}\right]
   &= \mathbb{E}\left[\log\left(\norm{\vect{y}-\vect{u}(t)}_2^2 \right)\right]-\mathbb{E}\left[\log(\norm{\vect{y}-\vect{u}(t)}^2)\right]\\
   &\leq  \mathbb{E}\left[\log \left( \norm{\vect{y}-\vect{u}(0)}_2^2\right) \right]<\infty
\end{align*}
Then $\{Z_t\}_{t=0}^{T}$ is a sub-martingale as $\mathbb{E}\left[Z_{t}\right]$  is finite for any $t$ and by inequality \eqref{eq:y-u1} 
\begin{align}
    &\mathbb{E}_{\xi_{t-1}}\left[Z_{t}\right] - Z_{t-1} \nonumber\\
  =  & \mathbb{E}_{\xi_{t-1}}\left[\log\left(\norm{\vect{y}-\vect{u}(t)}_2^2  \right)\right] - \mathbb{E}_{\xi_{t-1}}\left[\log(\norm{\vect{y}-\vect{u}(t+1)}^2)\right] - \log\left( 1-\frac{\eta \lambda_0}{2n}\right) \nonumber\\
  \leq &0\nonumber
%   \leq   &\log(\norm{\vect{y}-\vect{u}(t)}^2)-C_1 - \mathbb{E}_{\xi_{t-1}}\left[\log(\norm{\vect{y}-\vect{u}(t)}^2)\right]\nonumber\\
%     \leq &Z_{t-1}.
\end{align}
In order to use and extended Azuma Inequality \cite{chung2006concentration,allen2018convergence,
zou2018stochastic}\footnote{Theorem 27 in \cite{chung2006concentration}}, we need to verify the condition
     \begin{align}
          \mathbb{E}_{\xi_{t-1}}\left[\left(Z_{t} - \mathbb{E}_{\xi_{t-1}}[Z_{t}]\right)^2\right]\leq \sigma_t^2\quad  \text{ and }\quad 
         Z_{t} - \mathbb{E}_{\xi_{t-1}}[Z_{t}]\leq c_t  \quad \text{for} \quad t \in [t+1]  .\label{eq:c-lip}
     \end{align}
 Bounding the random variable $\norm{\vect{u}(t+1)-\vect{u}(t)}_2^2$ with no expectation, we get %\eqref{eq:defineUU}, we b
\begin{align}
\norm{\vect{u}(t+1)-\vect{u}(t)}_2^2
&= \sum_{i=1}^n\left(u_i(t+1)-u_i (t) \right)^2 \nonumber\\
&\leq \eta^2 \sum_{i=1}^n \sum_{r=1}^m\abs{\bigg \langle{ \frac{\partial L_{\xi_t}(\mat{W}(t))}{\partial \vect{w}_r(t)}, \vx_i \bigg\rangle}}^2 \nonumber\\
&\leq  \eta ^2 n|y_{\xi_t}-u_{\xi_t}(t)|^2 \nonumber\\
&\le  \eta^2 n \|\vy-\vu(t)\|^2. 
\end{align}
Therefore, we have
\begin{align}
\norm{\vect{y}-\vect{u}(t+1)} = & \norm{\vect{y}-\vect{u}(t) - (\vect{u}(t+1)-\vect{u}(t))}\nonumber\\
= & \norm{\vect{y}-\vect{u}(t)}+ \norm{\vect{u}(t+1)-\vect{u}(t)} \nonumber\\
% \leq & \norm{\vect{y}-\vect{u}(t)} + \norm{\vect{u}(t+1)-\vect{u}(t)}\left(\norm{\vect{u}(t+1)-\vect{u}(t)}+ 2 \|\vect{y}-\vect{u}(t)\| \right)\nonumber\\
% \leq & \norm{\vect{y}-\vect{u}(t)}^2+\eta\sqrt{n} \max_{j\in[n]} |y_{j}-u_{j}(t)|\left(\norm{\vect{y}-\vect{u}(t)}  + 2\eta\sqrt{n} \max_{j\in[n]} |y_{j}-u_{j}(t)|\right) \nonumber\\
\le & \left(1+ \eta \sqrt{n} \right)\norm{\vect{y}-\vect{u}(t)}\nonumber\\
\Rightarrow \quad\log \left(\norm{\vect{y}-\vect{u}(t+1)}^2\right) &\leq \log\left(\norm{\vect{y}-\vect{u}(t)}^2\right) +2\log \left( 1+ \eta \sqrt{n} \right)  \label{eq:right}
% \\
% \Rightarrow \quad & Z_{t+1}\leq Z_{t}+ C_1\nonumber \\ 
\end{align} 
With the learning rate $\eta \leq\frac{\lambda_0}{n}< \frac{1}{\sqrt{n}}$,
\begin{align}
\norm{\vect{y}-\vect{u}(t)}
= &  \norm{\vect{y}-\vect{u}(t+1) - (\vect{u}(t+1)-\vect{u}(t))}\nonumber\\
\leq &  \norm{\vect{y}-\vect{u}(t+1)} + \|\vect{u}(t+1)-\vect{u}(t))\|\nonumber \\
\le & \frac{1 }{1-\eta \sqrt{n}}\norm{\vect{y}-\vect{u}(t+1)}\nonumber\\
\Rightarrow \quad\log \left(\norm{\vect{y}-\vect{u}(t)}^2\right) &\leq \log\left(\norm{\vect{y}-\vect{u}(t+1)}^2\right) +2\log \left(\frac{1}{1-\eta\sqrt{n}} \right) \label{eq:left}
% \\
% \Rightarrow \quad & Z_{t+1}\leq Z_{t}+ C_2\nonumber
\end{align}
Thus combining \eqref{eq:left} and \eqref{eq:right} gives
$$|Z_{t}-Z_{t-1}|=\abs{ \log\left(\norm{\vect{y}-\vect{u}(t+1)}^2\right) - \log\left(\norm{\vect{y}-\vect{u}(t)}^2\right)} \leq 2\log \left(\frac{1}{1-\eta\sqrt{n}} \right)$$
We now verify condition \eqref{eq:c-lip} as follows for $t\in[T]$
\begin{align*}
\mathbb{E}_{\xi_{t-1}}\left[\left(Z_{t} - \mathbb{E}_{\xi_{t-1}}[Z_{t}]\right)^2\right] =& \mathbb{E}_{\xi_{t-1}}\left[\left(Z_{t} - Z_{t-1} - \mathbb{E}_{\xi_{t-1}}[Z_{t}-Z_{t-1}]\right)^2\right]\\
\leq & \mathbb{E}_{\xi_{t-1}}\left[\left(Z_{t} - Z_{t-1} \right)^2\right]- \left(\mathbb{E}_{\xi_{t-1}}[Z_{t}-Z_{t-1}]\right)^2\\
\leq &  4 \log^2 \left(\frac{1}{1-\eta\sqrt{n}} \right) \\
 Z_{t} - \mathbb{E}_{\xi_{t-1}}[Z_{t}]\leq  2\log \left(\frac{1}{1-\eta\sqrt{n}} \right) &- \mathbb{E}_{\xi_{t-1}}[Z_{t}-Z_{t-1} ] \leq 4 \log \left(\frac{1}{1-\eta\sqrt{n}} \right)
\end{align*} 
Thus, we have  with probability $$1-\exp\left(\frac{32t\log^2\left(n \right)\log^2\left(\frac{1}{1-\eta \sqrt{n}}\right)}{32t\log^2\left(\frac{1}{1-\eta \sqrt{n}}\right) + 4\sqrt{t}\log^2\left(\frac{1}{1-\eta \sqrt{n}}\right)\log\left(n \right)/3  }  \right)=1-e^{ \Omega \left(\log^2(n)\right) },$$
we have 
\begin{align*}
    Z_t  &\leq Z_0+ 4\sqrt{2t} \log\left(\frac{1}{1-\eta \sqrt{n}}\right)\log\left(n \right)\\
 \Rightarrow \quad & \log\left(\norm{\vect{y}-\vect{u}(t)}^2 \right)\\
 \leq & t\log\left(1-\frac{\eta \lambda_0}{2n}\right)+\log\left(\norm{\vect{y}-\vect{u}(0)}^2 \right) + 4\sqrt{2t} \log\left(\frac{1}{1-\eta \sqrt{n}}\right)\log\left(n \right) \\
 \leq & \log\left(\norm{\vect{y}-\vect{u}(0)}^2 \right) + 4\sqrt{2t} \log\left(\frac{1}{1-\eta \sqrt{n}}\right)\log\left(n \right) +t\log\left(1-\frac{\eta \lambda_0}{2n}\right)
\end{align*}


\end{proof}



